Weighted Context-Free-Language Ordered Binary Decision Diagrams

This paper presents a new data structure, called \emph{Weighted Context-Free-Language Ordered BDDs} (WCFLOBDDs), which are a hierarchically structured decision diagram, akin to Weighted BDDs (WBDDs) enhanced with a procedure-call mechanism. For some functions, WCFLOBDDs are exponentially more succinct than WBDDs. They are potentially beneficial for representing functions of type $\mathbb{B}^n \rightarrow D$, when a function's image $V \subseteq D$ has many different values. We apply WCFLOBDDs in quantum-circuit simulation, and find that they perform better than WBDDs on certain benchmarks. With a 15-minute timeout, the number of qubits that can be handled by WCFLOBDDs is 1-64$\times$ that of WBDDs (and 1-128$\times$ that of CFLOBDDs, which are an unweighted version of WCFLOBDDs). These results support the conclusion that for this application -- from the standpoint of problem size, measured as the number of qubits -- WCFLOBDDs provide the best of both worlds: performance roughly matches whichever of WBDDs and CFLOBDDs is better. (From the standpoint of running time, the results are more nuanced.)

==> algos.tex <==
\section{Operations on WCFLOBDDs}
\label{Se:algos}

\begin{figure}[tb!]
    \centering
    \includegraphics[scale=0.44]{figures/walsh1-rep.pdf}
    \caption{Object-oriented representation of the WCFLOBDD for Hadamard matrix $H$ from~\figref{wcflobdd_hadamard}.}
    \label{Fi:oops_wcflobdd}
    \vspace{-3ex}
\end{figure}

This section describes the algorithms for operations on WCFLOBDDs. Because WCFLOBDDs are hierarchical structures, the algorithms are inspired by the algorithms for CFLOBDDs~\cite{DBLP:journals/corr/abs-2302-04349}. 
However, because WCFLOBDDs involve weights at level-$0$ groupings, the algorithms, along with respecting the hierarchical structure,
\twrchanged{
must also ensure the weights are handled properly so that the structural invariants hold.
}
Algorithms are given using an object-oriented pseudo-code.
\figref{oops_wcflobdd} shows the object-oriented representation of the WCFLOBDD for matrix $H_2$ from \figref{wcflobdd_hadamard}(a). There are three grouping classes:
$\texttt{InternalGrouping}$, $\texttt{ForkGrouping}$, and $\texttt{DontCareGrouping}$.
The latter two are level-$0$ groupings, which store left and right edge weights $(lw, rw)$.
Operations that construct a $\texttt{ForkGrouping}$ or a $\texttt{DontCareGrouping}$ take two inputs, $lw$ and $rw$.
All groupings at levels $\geq 1$ are $\texttt{InternalGrouping}$s.

% \twrchanged{
Our algorithms use two standard techniques (mostly elided in the pseudo-code).
\emph{Hash consing}~\cite{goto1974monocopy} is used to ensure that only one representative of a value exists in memory.
The operation ${\tt RepresentativeGrouping }$ checks whether a grouping is a duplicate, and if so, discards it and returns the grouping's representative.
Consequently, we can test in unit time if two proto-WCFLOBDDs are equal by comparing their pointers.
\Omit{
    This ability allows some special cases to be identified quickly (\sectref{primitiveops}), and helps speed up computations.
}
A \emph{cache} for a function $F$ is an associative-lookup table with pairs of the form $[x, F(x)]$, used to eliminate the cost of re-doing a previously performed computation \cite{michie1967memo}.
% }

\subsection{Constant Functions}
\label{Se:primitiveops}

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/noDistinction1.pdf}
    \caption{Level-$1$ ConstantOneProtoCFLOBDD}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/noDistinctionAnn1.pdf}
    \caption{Level-$1$ ConstantZeroProtoCFLOBDD}
    \end{subfigure}
\Omit{
    \begin{subfigure}{0.22\linewidth}
    \includegraphics[width=.8\linewidth]{figures/noDistinction2.pdf}
    \caption{Level-$2$ ConstantOneProtoCFLOBDD}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=.8\linewidth]{figures/noDistinctionAnn2.pdf}
    \caption{Level-$2$ ConstantZeroProtoCFLOBDD}
    \end{subfigure}
}
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/noDistinctionK.pdf}
    \caption{Level-$k$ ConstantOneProtoCFLOBDD}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/noDistinctionAnnK.pdf}
    \caption{Level-$k$ ConstantZeroProtoCFLOBDD}
    \end{subfigure}
\caption{${\tt ConstantOneProtoCFLOBDD }$ and ${\tt ConstantZeroProtoCFLOBDD}$ for levels $1$\Omit{, $2$,} and $k > 1$.}
\label{Fi:nodistinctfigs}
\vspace{-4ex}
\end{figure}

\begin{algorithm}[tb!]
\caption{ConstantZeroProtoCFLOBDD\label{Fi:ConstantZeroProtoCFLOBDDAlgorithm}}
\small{
\Input{int k -- level of the topmost grouping}
\Output{Proto-CFLOBDD for $\lambda x. \bar{0}$ with $2^k$ variables}
\Begin{
\lIf{k == 0}{\Return RepresentativeDontCareGrouping($\bar{0},\bar{0}$)}
InternalGrouping g = new InternalGrouping(k)\;
g.AConnection = ConstantZeroProtoCFLOBDD(k-1)\;
g.AReturnTuple = [1]\;
g.numberOfBConnections = 1\;
g.BConnections[1] = g.AConnection\;
g.BReturnTuples[1] = [1]\;
g.numberOfExits = 1\;
\Return RepresentativeGrouping(g)\;
}
}
\end{algorithm}

\Omit{
\begin{algorithm}
\caption{ConstantOneProtoCFLOBDD\label{Fi:ConstantOneProtoCFLOBDDAlgorithm}}
\small{
\Input{int k -- level of the topmost grouping}
\Output{Proto-CFLOBDD for $\lambda x. \bar{1}$ with $2^k$ variables}
\Begin{
\If{k == 0}{\Return RepresentativeDontCareGrouping(1,1)\;}
InternalGrouping g = new InternalGrouping(k)\;
g.AConnection = ConstantOneProtoCFLOBDD(k-1)\;
g.AReturnTuple = [1]\;
g.numberOfBConnections = 1\;
g.BConnections[1] = g.AConnection\;
g.BReturnTuples[1] = [1]\;
g.numberOfExits = 1\;
\Return RepresentativeGrouping(g)\;
}
}
\end{algorithm}
}

\figref{nodistinctfigs} shows the $\protoWCFLOBDD$s for the constant functions $f_{\bar{0}}(x) = \lambda x. \bar{0}$ and $ f_{\bar{1}}(x) = \lambda x. \bar{1}$ (also called $\texttt{ConstantZero}$ and $\texttt{ConstantOne}$, respectively).
These $\protoWCFLOBDD$s each have just one kind of level-$0$ grouping.
The value tuples for $f_{\bar{0}}$ and $f_{\bar{1}}$ are $[\bar{0}]$ and $[\bar{1}]$, respectively.
\algref{ConstantZeroProtoCFLOBDDAlgorithm} gives pseudo-code to create the $\protoWCFLOBDD$ of $\texttt{ConstantZero}$;
$\texttt{ConstantOne}$ is similar.
\Omit{Many WCFLOBDDs algorithms perform equality tests on groupings with $\texttt{ConstantZero}$ and $\texttt{ConstantOne}$ to identify arguments on which to perform special-case handling.}

\subsection{Unary Operations}
\emph{Scalar Multiplication.} Given a scalar value $v \in \mathcal{D}$ and the WCFLOBDD $C = \langle \textit{fw}, g, \textit{vt} \rangle$ for a function $f$,
% \twrchanged{
the WCFLOBDD $C'$ for the function $\lambda x. (v \cdot f(x))$ is
\[
  C' = \begin{cases}
         \langle v \cdot \textit{fw}, g, \textit{vt} \rangle & v \neq \bar{0} \\
         \texttt{ConstantZero} & v = \bar{0}
       \end{cases}
\]
% }
% algorithm ${\tt ScalarMultiplyCFLOBDD }$ of~\algref{ScalarMultiplyCFLOBDDAlgorithm} shows the operation of performing the multiplication of $v$ with $C$. If $v$ is $\bar{0}$, then a ${\tt ConstantZero }$ is returned, else a new WCFLOBDD $C' = \langle v \cdot fw, g, vt \rangle$ is returned.

% \begin{algorithm}
% \small{
% \Input{CFLOBDD c = $\langle fw, g, vt \rangle$, Value v}
% \Output{CFLOBDD c' = v $\ast$ c}
% \Begin{
% \If{v == $\bar{0}$}{\Return ConstantZeroProtoCFLOBDD(c.level)\;}
% \Return RepresentativeCFLOBDD(g, vt, v $\cdot$ fw)\;
% }
% }
% \caption{ScalarMultiplyCFLOBDD\label{Fi:ScalarMultiplyCFLOBDDAlgorithm}}
% \end{algorithm}

\subsection{Pointwise Binary Operations}
% \twrchanged{
A binary operation $\op$ works \emph{pointwise} if, for two functions $f$ and $g$, $f \op g \eqdef \lambda x . f(x) \op g(x)$.
We discuss $\op \in \{ \cdot, + \}$.
% }

\subsubsection{Pointwise Multiplication.}
Given $f$ and $g$, compute $f \cdot g$. 

\iffalse
\begin{algorithm}[tb!]
\caption{Multiplicative Binary Operation (MBO)}
\Input{CFLOBDDs $c_1 = \langle fw_1, g_1, v_1 \rangle , c_2 = \langle fw_2, g_2, v_2 \rangle$}
\Output{CFLOBDD $c = c_1 \cdot c_2$}
\tcp{Perform cross product}
Grouping$\times$Tuple $[g, pt]$ = MulPairProduct($g_1$, $g_2$)\;
ValueTuple $v$ = $[v_1[i_1] \cdot v_2[i_2] : [i_1, i_2] \in pt]$\;
Tuple$\times$Tuple [returnTuple, reductionTuple] = CollapseClasses($v$)\;
Grouping $g'$ = Reduce($g$, reductionTuple, $v$)\;
\Return RepresentativeWCFLOBDD($g'$, returnTuple, $fw_1 \cdot fw_2$)\;
\end{algorithm}

\begin{algorithm}[tb!]
\caption{MulPairProduct}
\Input{Groupings $g_1, g_2$}
\Output{Grouping $g = g_1 \cdot g_2$}

    \If {$g_1$ and $g_2$ are both no-distinction groupings with weight $\bar{1}$}
    { \Return [ $g_1$, [[1,1]] ]\;}   
    \If {$g_1$ is a no-distinction grouping with weight $\bar{1}$}
    {\Return [ $g_2$, [[1,k]~:~k $\in$ [1..$g_2$.numberOfExits]] ] \;}
    \If {$g_2$ is a no-distinction grouping with weight $\bar{1}$}
    {\Return [ $g_1$, [[k,1]~:~k $\in$ [1..$g_1$.numberOfExits]] ]\;}
    \If {$g_1$ and $g_2$ are both fork groupings} 
    {\Return [ $g_1$, [[1,1],[2,2]] ]\;} 

\tcp{Cross product on A-Connections}
Grouping$\times$Tuple $[gA, ptA]$ = MulPairProduct($g_1.$AConnection, $g_2$.AConnection)\;
InternalGrouping $g$ = new InternalGrouping($g_1$.level)\;
$g$.AConnection = $gA$\;
$g$.AReturnTuple = $[1..|ptA|]$\;
$g$.numberOfBConnections = $|ptA|$\;

Tuple ptAns = []\;

    \tcp{Create a B-connection for each middle vertex}
    \For {$j \leftarrow 1$ \KwTo $|ptA|$}{
        Grouping$\times$PairTuple $[gB,ptB]$ = MulPairProduct($g_1$.BConnections[$ptA$(j)(1)], $g_2$.BConnections[$ptA$(j)(2)])\;
        $g$.BConnections[j] = $gB$ \;
        \tcp{Now create g.BReturnTuples[j], and augment ptAns as necessary}
        $g$.BReturnTuples[j] = [] \;        \label{Li:PPExitVertexLoopStart}
        \For{$i \leftarrow 1$ \KwTo $|ptB|$} {
            $n_1$ = $g_1$.BReturnTuples[$ptA$(j)(1)]($ptB$(i)(1))\tcp*[r]{an exit vertex of $g_1$}
            $n_2$ = $g_2$.BReturnTuples[$ptA$(j)(2)]($ptB$(i)(2)) \tcp*[r]{an exit vertex of $g_2$}
            \eIf(\tcp*[f]{Not a new exit vertex of $g$}){[$n_1,n_2$] $\in$ $ptAns$}
                {
                index = the k such that $ptAns(k)$ == $[n_1,n_2]$ \;
                $g$.BReturnTuples[j] = $g$.BReturnTuples[j] || index \;
                }
            (\tcp*[f]{Identified a new exit vertex of g}){
                $g$.numberOfExits = $g$.numberOfExits + 1 \;
                $g$.BReturnTuples[j] = $g$.BReturnTuples[j] $||$ $g$.numberOfExits \;
                $ptAns = ptAns || [n_1,n_2]$ \;
            }
        }  
    }
    \Return [RepresentativeGrouping($g$), $ptAns$]\;
\end{algorithm}
\fi

Let $c_1 = \langle \textit{fw}_1, g_1, v_1\rangle$ and $c_2 = \langle \textit{fw}_2, g_2, v_2 \rangle$ be the WCFLOBDDs that represent $f$ and $g$, respectively.
% \twrchanged{
As with BDDs, such operations on WCFLOBDDs can be implemented via a two-step process:
(i) create a cross-product of $c_1$ and $c_2$, and
(ii) perform a reduction step on the result of step (i).
% }
The cross-product is performed recursively on the A-Connection groupings, followed by the B-Connection groupings.
% \twrchanged{
The cross-product of two groupings yields a tuple of the form ($g$, $[pt]$), where $g$ is the resultant grouping and $pt$ is a sequence of index-pairs.
The index-pairs in $pt$ indicate the B-Connection groupings on which cross-product operations need to be performed.
\figref{PairProductIllustraction} shows the cross-product of the WCFLOBDDs that represent
$H_2 = \frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
        1 & 1\\
        1 & -1
    \end{smallmatrix}\right]$
and $I_2 = \left[\begin{smallmatrix}
        1 & 0\\
        0 & 1\\
        \end{smallmatrix}\right]$.
% }

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/mob_1.pdf}
        \caption{$H_2 = \frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
        1 & 1\\
        1 & -1
    \end{smallmatrix}\right]$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/mob_2.pdf}
        \caption{$I_2 = \left[\begin{smallmatrix}
        1 & 0\\
        0 & 1\\
        \end{smallmatrix}\right]$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/mob_3.pdf}
        \caption{Result of ${\tt PairProduct}$ on (a) and (b)}
    \end{subfigure}
    \caption{Illustration of ${\tt PairProduct}$ on two functions.}
    \label{Fi:PairProductIllustraction}
    \vspace{-3ex}
\end{figure}

At level-$0$ and the topmost level, the algorithm performs:
\begin{itemize}
  \item
    Level-$0$:
    Let the two level-$0$ groupings be $g_1^0$ with weights $(lw_1, rw_1)$ and $g_2^0$ with weights $(lw_2, rw_2)$.
    The return value is a new level-$0$ grouping $g$, with weights $(lw_1 \cdot lw_2, rw_1 \cdot rw_2)$, along with a sequence of index-pairs on which the cross-product is performed next.
    For example, if $g_1^0$ is a fork-grouping and $g_2^0$ is a don't-care grouping, then $pt = [(1,1), (2,1)]$.
  \item
    Topmost level:
    If $(g, pt)$ is returned after performing the cross-product, the indices in $pt$ are indices into the value tuples of $c_1$ and $c_2$.
% \twrchanged{
    A new value tuple $v$ is constructed accordingly.
    For instance, if $v_1 = [\bar{1}, \bar{0}]$, $v_2 = [\bar{0}, \bar{1}]$, and $pt = [(1,1), (1, 2), (2, 1)]$, then $v$ is
    $[ (v_1[1] \cdot v_2[1]), (v_1[1] \cdot v_2[2]), (v_1[2] \cdot v_2[1])] = [\bar{1} \cdot \bar{0}, \bar{1} \cdot \bar{1}, \bar{0} \cdot \bar{0}] = [\bar{0}, \bar{1}, \bar{0}]$.
% }
\end{itemize}



% \twrchanged{
When the resulting value tuple has duplicate entries, such as $v = [\bar{0}, \bar{1}, \bar{0}]$ in the example above, it is necessary to perform a reduction step, \texttt{Reduce}, to maintain the WCFLOBDD structural invariants.
In this case, \texttt{Reduce} folds together the first and third exit vertices of $g$, which are both mapped to $\bar{0}$ by $v$.
In \algref{MBO}, the information that directs the reduction step is obtained by calling CollapseClassesLeftmost (\algref{InducedTuples}), which returns two tuples:
inducedValueTuple (here, $[\bar{0}, \bar{1}]$) and inducedReductionTuple (here, $[1, 2, 1]$):
inducedValueTuple consists of the leftmost occurrences of $\bar{0}$ and $\bar{1}$ in $v$, in the same left-to-right order in which they occur in $v$;
inducedReductionTuple indicates where each occurrence of $\bar{0}$ and $\bar{1}$ in $v$ is mapped to in inducedValueTuple.
\texttt{Reduce} traverses $g$ backwards to create $g'$, a reduced version of $g$ that, together with inducedValueTuple as its terminal values, satisfies the WCFLOBDD structural invariants.
% Optimizations such as function caching and computations for special cases such as ${\tt ConstantZero}$ and ${\tt ConstantOne}$ can be performed without traversing all the levels of the groupings.
The result from $c_1 \cdot c_2$ is the WCFLOBDD $\langle \textit{fw}_1 \cdot \textit{fw}_2, g', \textrm{inducedValueTuple} \rangle$.
% }

Just as there can be multiple occurrences of a given node in a BDD, there can be multiple occurrences of a given grouping in a WCFLOBDD.
To avoid a blow-up in costs, binary operations need to avoid making repeated calls on a given pair of groupings $h_1 \in c_1$ and $h_2 \in c_2$.
Assuming that the hashing methods used for hash-consing and function caching run in expected unit-cost time, the cost of the ``cross-product'' is bounded by the product of the sizes of the two-argument WCFLOBDDs. 
\mas{However, the cost of {\tt Reduce} is bounded by the product of the sizes of the input and output WCFLOBDDs.}

The pseudocode is shown in~\algref{MBO}, which calls~\algref{PairProduct} \mas{(analogous to the product construction in BDDs and FSMs)} and~\algref{Reduce} \mas{(analogous to the Reduce operation in BDDs)}, which in turn call~\algrefs{InducedTuples}{InsertBConnection}.
\begin{itemize}
  \item
    \algref{PairProduct} recursively perform the cross-product on input groupings $g1$, $g2$ to form a new grouping $g$, along with $pt$, which is a tuple of exit-vertex pairs.
  \item
    \algref{InducedTuples} collapses $pt$ to enforce structual invariants on the value tuple.
  \item
% \twrchanged{
    \algref{Reduce} reduces a grouping based on return tuples or the value tuple, and as a by-product ensures canonicity of the resulting WCFLOBDD (see  \sectref{AlgorithmsUsedInPointwiseMultiplication}).
% }
  \item
% \twrchanged{
    \algref{InsertBConnection} determines the position for a B-Connection in a grouping being constructed, reusing one if it is already present in the grouping (see  \sectref{AlgorithmsUsedInPointwiseMultiplication}).
% }
\end{itemize}

\subsubsection{Pointwise Addition.}

Given $f$ and $g$, compute $f + g$.
The algorithm, in \sectref{PointwiseAddition}, is similar to pointwise multiplication.

\begin{algorithm}
\small{
\Input{WCFLOBDDs n1 = $\langle \textit{fw1}, g1, \textit{vt1} \rangle$, n2 = $\langle \textit{fw2}, g2, \textit{vt2} \rangle$}
\Output{CFLOBDD n = n1 $\cdot$ n2}
\Begin{
\tcp{Perform cross product}
    Grouping$\times$PairTuple [g,pt] = PairProduct(g1,g2)\;  \label{Li:BAAR:CallPairProduct}
    ValueTuple deducedValueTuple = [ vt1[i1] $\cdot$ vt2[i2]~:~[i1,i2] $\in$ pt ]\;  \label{Li:BAAR:LeafValues}
     \tcp{Collapse duplicate leaf values, folding to the left}
    Tuple$\times$Tuple [inducedValueTuple,inducedReductionTuple] = CollapseClassesLeftmost(deducedValueTuple)\;  \label{Li:BAAR:CollapseLeafValues}
    Grouping$\times$Weight [g', $\textit{fw}$] = Reduce(g, inducedReductionTuple, deducedValueTuple)\;  \label{Li:BAAR:CallReduce}
    WCFLOBDD n = RepresentativeCFLOBDD($\textit{fw} \cdot \textit{fw1} \cdot \textit{fw2}$, g', inducedValueTuple)\;
    \Return n\;
}
}
\caption{Pointwise Multiplication\label{Fi:MBO}}
\end{algorithm}

\begin{algorithm}[tb!]
\caption{PairProduct\label{Fi:PairProduct}}
\small{
\Input{Groupings g1, g2}
\Output{Grouping g: product of g1 and g2; PairTuple ptAns: tuple of pairs of exit vertices}
\SetKwBlock{Begin}{Begin}{}
\Begin{
    \lIf {g1 and g2 are both ConstantOneProtoCFLOBDD \label{Li:PPConstantOneStart}}  
    { \Return [ g1, [[1,1]] ]}   
    \lIf {g1 or g2 is ConstantZeroProtoCFLOBDD }  
    { \Return [ ConstantZeroProtoCFLOBDD(g1.level), [[1,1]] ]}   
    \lIf {g1 is ConstantOneProtoCFLOBDD}
    {\Return [ g2, [[1,k]~:~k $\in$ [1..g2.numberOfExits]] ]}
    \lIf {g2 is ConstantOneProtoCFLOBDD}
    {\Return [ g1, [[k,1]~:~k $\in$ [1..g1.numberOfExits]] ]}      \label{Li:PPConstantOneEnd}
\tcp{Similar cases for other base cases, with appropriate pairings of exit vertices}
\If {g1 and g2 are fork groupings  \label{Li:PPBothForkGroupings}} {
    ForkGrouping g = new ForkGrouping(g1.lw $\cdot$ g2.lw, g1.rw $\cdot$ g2.rw)\;
\Return [ g, [[1,1],[2,2]] ]\;
} \label{Li:PPBothForkGroupingsEnd}
\tcp{ Pair the A-connections}
    Grouping$\times$PairTuple [gA,ptA] = PairProduct(g1.AConnection, g2.AConnection)\;
    InternalGrouping g = new InternalGrouping(g1.level)\;
    g.AConnection = gA\;
    g.AReturnTuple = [1..$|$ptA$|$]\tcp*[r]{Represents the middle vertices}
    g.numberOfBConnections = $|$ptA$|$\;  \label{Li:PPNumberOfBConnections}
    \tcp{Pair the B-connections, but only for pairs in ptA }
    \tcp{Descriptor of pairings of exit vertices}
    Tuple ptAns = []\;  \label{Li:ptAnsDeclaration}

    \tcp{Create a B-connection for each middle vertex}
    \For {$j \leftarrow 1$ \KwTo $|ptA|$}{
        Grouping$\times$PairTuple [gB,ptB] = PairProduct(g1.BConnections[ptA(j)(1)], g2.BConnections[ptA(j)(2)])\;
        g.BConnections[j] = gB \;
        \tcp{Create g.BReturnTuples[j], and augment ptAns as necessary}
        g.BReturnTuples[j] = [] \;        \label{Li:PPExitVertexLoopStart}
        \For{$i \leftarrow 1$ \KwTo $|ptB|$} {
            c1 = g1.BReturnTuples[ptA(j)(1)](ptB(i)(1))\tcp*[r]{a g1 exit}
            c2 = g2.BReturnTuples[ptA(j)(2)](ptB(i)(2)) \tcp*[r]{a g2 exit}
            \eIf(\tcp*[f]{Not a new exit vertex of g}){[c1,c2] $\in$ ptAns}
                {
                index = the k such that ptAns(k) == [c1,c2] \;
                g.BReturnTuples[j] = g.BReturnTuples[j] $||$ index \;
                }
            (\tcp*[f]{Identified a new exit vertex of g}){
                g.numberOfExits = g.numberOfExits + 1 \;
                g.BReturnTuples[j] = g.BReturnTuples[j] $||$ g.numberOfExits \;
                ptAns = ptAns $||$ [c1,c2] \; \label{Li:PPConcatenateExitPair}
            }
        }  \label{Li:PPExitVertexLoopEnd}
    }
    \Return [RepresentativeGrouping(g), ptAns]\; \label{Li:PPTabulateAnswer}
}
}
\end{algorithm}


\begin{algorithm}
\caption{CollapseClassesLeftmost\label{Fi:InducedTuples}}
\small{
\Input{Tuple equivClasses}
\Output{Tuple$\times$Tuple [projectedClasses, renumberedClasses]}
\Begin{
\tcp{Project the tuple equivClasses, preserving left-to-right order, retaining the leftmost instance of each class}
\label{Li:IT:TupleCollapseStart}
Tuple projectedClasses = [equivClasses(i) : i $\in$ [1..$|$equivClasses$|$] $|$ i = min\{j $\in$ [1..$|$equivClasses$|$] $|$ equivClasses(j) = equivClasses(i)\}]\;
\label{Li:IT:TupleCollapseEnd}
\tcp{Create tuple in which classes in equivClasses are renumbered according to their ordinal position in projectedClasses}
Map orderOfProjectedClasses = \{[x,i]: i $\in$ [1..$|$projectedClasses$|$] $|$ x = projectedClasses(i)\}\;
Tuple renumberedClasses = [orderOfProjectedClasses(v) : v $\in$ equivClasses]\;
\Return [projectedClasses, renumberedClasses]\;
}
}
\end{algorithm}


\subsection{Representing Matrices and Vectors}
% In this subsection and the next three, we discuss how to represent matrices and vectors using WCFLOBDDs and perform some important operations on them.

% \twrchanged{
When matrices are represented with WCFLOBDDs, the variables correspond to the bits of the matrix's row and column indices.
% }
For a matrix $M$ of size $2^{n} \times 2^{n}$, the WCFLOBDD representation has $2n$ variables $(x_0, \ldots, x_{n-1})$ and $(y_0, \ldots, y_{n-1})$, where the $x$-variables are the row bits and $y$-variables are the column bits.
Typically, we use a variable ordering in which the $x$ and $y$ variables are interleaved.
The nice property of this ordering is that, as we work through each pair of variables in an assignment, the matrix elements that remain ``in play'' represent a sub-block of $M$. 

% \twrchanged{
When vectors of size $2^n \times 1$ are represented using WCFLOBDDs, the variables $(x_0, \ldots, x_{n-1})$ correspond to the bits of the vector's row index.
% }
Typically, the ascending ordering of variables is used to represent vectors.

\input{matrix-multiplication}

See \sectrefs{KroneckerProduct}{Sampling} for algorithms for Kronecker product and sampling.



==> back.tex <==
\section{Background}
\label{Se:back}

% This section reviews BDDs, CFLOBDDs, and WBDDs, and briefly introduces the application area of quantum simulation.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[width=0.7\linewidth]{figures/walsh1_bdd_new.pdf}
    \caption{BDD}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[width=0.7\linewidth]{figures/walsh1.pdf}
    \caption{CFLOBDD}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[width=0.7\linewidth]{figures/walsh1_wbdd.pdf}
    \caption{WBDD}
    \end{subfigure}
    \caption{(a) BDD, (b) CFLOBDD, and (c) WBDD for the Hadamard matrix $\frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
    1 & 1\\
    1 & -1
    \end{smallmatrix}\right]$,
    with the variable ordering $\langle x_0, y_0 \rangle$ ($x_0$, $y_0$: row, column variables).
    }
    \label{Fi:data-structures}
    \vspace{-3ex}
\end{figure}

\subsection{Binary Decision Diagrams (BDDs)}
Binary Decision Diagrams (BDDs) \cite{toc:Bryant86} are data structures used to efficiently represent functions from Boolean variables to Boolean or non-Boolean values.\footnote{
  BDDs with a non-Boolean range are called MTBDDs \cite{DBLP:journals/fmsd/FujitaMY97} or ADDs \cite{DBLP:journals/fmsd/BaharFGHMPS97}.
  We use ``BDD'' as a generic term for both BDDs and MTBDDs/ADDs.
}
Every node in a BDD corresponds to a decision variable and the outgoing edges of every node correspond to the variable's decision, $0$ or $1$.\footnote{
  In all diagrams, left branches are for $0$ ($F$); right branches are for $1$ ($T$).
}
The terminal values or ``leaves" of the BDD represent the unique values of the function's output. In the best case, BDDs provide exponential compression over the decision-tree representation of the function.~\figref{data-structures}(a) shows the BDD representation for Hadamard matrix $\frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
    1 & 1\\
    1 & -1
    \end{smallmatrix}\right]$
with variable ordering $\langle x_0, y_0 \rangle$, where $x_0$ is the row decision variable and $y_0$ is column decision variable. The highlighted path shows the assignment $\{ x_0 \mapsto 1, y_0 \mapsto 1\}$, which evaluates to $H[1][1] = \frac{-1}{\sqrt{2}}$.

\subsection{Context-Free-Language Ordered Binary Decision Diagrams (CFLOBDDs)}
% CFLOBDDs  are data structures inspired by BDDs but based on different principles. 
\mas{
CFLOBDDs \cite{DBLP:journals/corr/abs-2211-06818} can be interpreted from an automata-theoretic or programming language perspective. (1) CFLOBDDs are a particular kind of \emph{single-entry, multi-exit hierarchical finite-state machines}, (2) can be considered as bounded-size, branching but non-looping programs with the allowance of a certain form of procedure calls.
}

\mas{
Comparing CFLOBDDs with BDDs, BDDs could be thought as acyclic, finite-state machines or bounded-size, branching programs.
}
% BDDs can be considered as acyclic, finite-state machines, %(modulo ply-skipping), 
% whereas CFLOBDDs \cite{DBLP:journals/corr/abs-2211-06818} are a particular kind of \emph{single-entry, multi-exit hierarchical finite-state machines}. Similar to BDDs, CFLOBDDs can be considered as bounded-size, branching but non-looping programs.
% % \twrchanged{
% However, in CFLOBDDs a certain form of procedure call is permitted.
% % }

% \twrchanged{
In the best case, CFLOBDDs are exponentially more succinct than BDDs, and double-exponentially more succinct than decision trees.
% }
\mas{
Considering every node (``grouping'' in case of CFLOBDDs) as procedures,
}
the extra level of compression of CFLOBDDs over BDDs is due to the reuse of ``procedures'':
the same ``procedure'' can be called multiple times at different call sites.
These ``procedure calls'' enable additional sharing of structure in CFLOBDDs.
Where BDDs share sub-DAGs, CFLOBDDs can share the ``middle of a DAG.''

\mas{
The decisions in the case of CFLOBDDs for $x_0$ and $y_0$ variables are taken in the upper-right (or ``\emph{fork grouping}'') and lower-right (or ``\emph{dont-care grouping}'').
}
% \twrchanged{
The ``procedure call'' concept is illustrated in~\figref{data-structures}(b), which shows the CFLOBDD for the Hadamard matrix.
% }
The path highlighted in bold corresponds to the assignment $\{ x_0 \mapsto 1, y_0 \mapsto 1\}$ evaluating to $H[1][1] = \frac{-1}{\sqrt{2}}$.
% \twrchanged{
The oval object to the upper-right (or ``\emph{fork grouping}'') is shared twice: once during the red-highlighted path fragment and again during the blue-highlighted path fragment.
The corresponding regions are outlined in the BDD in~\figref{data-structures}(a)
\mas{
, where no sharing of nodes is observed.
}
% }

\mas{
Note that variables are not assigned to the decision nodes (``groupings'') in the case of CFLOBDDs.
Because of sharing at all levels, a given decision node does not represent a specific variable.
It is based on the following principle discussed in~\cite{DBLP:journals/corr/abs-2302-04349}.
}
\paragraph{Contextual-Interpretation Principle:} A level-0 grouping is not associated with a specific Boolean variable. Instead, the variable that a level-0 grouping refers to is determined by the context: the $n^{th}$ level-0 grouping visited along a matched path is used to interpret the $n^{th}$ Boolean variable.


\subsection{Weighted Binary Decision Diagrams (WBDDs)}
Weighted Binary Decision Diagrams (WBDDs) are extensions to BDDs with weights assigned to the decision edges.
% \twrchanged{
For a given assignment $a$ for a function $f$, $f(a)$ is computed by multiplying the weights encountered along the path for $a$.
% }

For example, consider the WBDD representation of the Hadamard matrix in~\figref{data-structures}(c). The weight $\frac{1}{\sqrt{2}}$ at the root of WBDD is common to all paths. The path highlighted in red corresponds to the assignment $\{ x_0 \mapsto 1, y_0 \mapsto 1\} = H[1][1] = \frac{1}{\sqrt{2}} * 1 * -1 = \frac{-1}{\sqrt{2}}$,
% \twrchanged{
where the weight for the decision $\{x_0 \mapsto 1 \}$ is $1$ and for $\{y_0 \mapsto 1\}$, when $\{x_0 \mapsto 1 \}$, is $-1$.
% }

To ensure canonicity, weights are scaled so that the weight of the left edge at every decision node is $1$.

\subsection{Quantum Simulation}
Quantum algorithms on quantum computers can achieve polynomial speed-ups over classical algorithms on specific problems.
% \twrchanged{
Simulation of quantum algorithms on classical machines allows researchers to experiment with quantum algorithms even without access to reliable quantum hardware.
Simulation uses a representation $qs$ of a quantum state, and performs gate applications and measurements on $qs$ via matrix multiplication and sampling, respectively.
% }

\Omit{
\twrchanged{
Simulation has several advantages.
For instance, some quantum algorithms perform multiple iterations of a particular quantum operator $\Op$ (e.g., $k$ iterations, where $k = 2^j$).
A simulation can operate on $\Op$ itself \cite[Ch.\ 6]{Book:ZW2020}, using $j$ iterations of repeated squaring to create matrices for $\Op^2$, $\Op^4, \ldots$, $\Op^{2^j} = \Op^k$.
% The final answer is then obtained using $\Op^k$.
In contrast, a physical device must apply $\Op$ sequentially, and thus performs $\Op$ $k = 2^j$ times.
}

\twrchanged{
Many quantum algorithms require multiple measurements on the final state.
After a measurement on a quantum computer, the quantum state collapses to the measured state.
Thus, every successive measurement requires re-running the quantum circuit.
However, with a simulation, the quantum state can be preserved across measurements, and thus the quantum circuit need only be executed once.
% \item Because quantum computers are error-prone and not fault-tolerant producing erroneous results, quantum simulation helps overcome this issue (module bugs in the implementation of the simulator).
% \item Quantum simulations can be used to develop test suites to verify the accuracy of outcomes obtained from measurements of quantum states on quantum hardware.
}
}

==> back2.tex <==
\section{Background}
\label{Se:back}

% This section reviews BDDs, CFLOBDDs, and WBDDs, and briefly introduces the application area of quantum simulation.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.2\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/walsh1_bdd_new.pdf}
    \caption{BDD for $H_2$}
    \end{subfigure}
    \begin{subfigure}{0.22\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/walsh1.pdf}
    \caption{CFLOBDD for $H_2$}
    \end{subfigure}
    \begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/walsh2_bdd_new.pdf}
    \caption{BDD for $H_4$}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/walsh2.pdf}
    \caption{CFLOBDD for $H_4$}
    \end{subfigure}
    \caption{(a) BDD and (b) CFLOBDD for the matrix $H_2$,
    with the ordering $\langle x_0, y_0 \rangle$ ($x_0$: row; $y_0$: column).
    (c) BDD and (d) CFLOBDD for the matrix $H_4$,
    with the ordering $\langle x_0, y_0, x_1, y_1 \rangle$ ($x_0, x_1$: row; $y_0, y_1$: column).
\twr{In (d) there is a missing red edge from $L_2$ entry to $L_1$ entry.}
    }
    \label{Fi:data-structures}
    \vspace{-3ex}
\end{figure}

\paragraph{BDDs.}
BDDs \cite{toc:Bryant86} are DAGs that represent functions from Boolean variables to Boolean or non-Boolean values.
Every node in a BDD corresponds to a decision variable and the outgoing edges of every node correspond to the variable's decision, $0$ or $1$.
\twrchanged{
The leaves of the BDD represent the values of the function's range.
}
In the best case, BDDs provide exponential compression over the decision-tree representation of the function.~\figref{data-structures}(a), and ~\figref{data-structures}(c) show the BDD representations for the first two matrices in $\mathcal{H}$, with interleaved $x$ and $y$ variables for rows and columns, respectively. The red paths show the all-$1$ assignments.

\paragraph{CFLOBDDs.}
% CFLOBDDs  are data structures inspired by BDDs but based on different principles. 
CFLOBDDs \cite{DBLP:journals/corr/abs-2211-06818} can be viewed from the perspective of
\twrchanged{
(i) automata theory, or (ii) programming languages; or
(i) a CFLOBDD is a particular kind of \emph{single-entry, multi-exit, non-recursive hierarchical finite-state machine};
(ii) a CFLOBDD is a bounded-size, branching but non-looping program, with a certain kind of non-recursive procedure call allowed.
}
In the best case, CFLOBDDs are exponentially more succinct than BDDs, and double-exponentially more succinct than decision trees.

\figref{data-structures}(b) and \figref{data-structures}(d) show the CFLOBDD representation for the first two matrices in $\mathcal{H}$. Because CFLOBDDs are hierarchical structures, different nodes in the CFLOBDD are divided into \emph{levels}.
\twrchanged{
A CFLOBDD at level $n$ represents a function of $2^n$ Boolean variables.
}
As seen in~\figref{data-structures}(b), the CFLOBDD represents matrix $H_2$ using two variables: $x_0$ (for row) and $y_0$ (for column), and has two levels: $L_0$ and $L_1$.

\twrchanged{
Each oval-shaped structure is called a \emph{grouping},
and is associated with a specific level.
A grouping at a level $\ge 1$ has a single entry vertex (black dot at the top), one or more middle vertices, and one or more exit vertices (at the bottom).
The three sets of vertices are disjoint.
\begin{itemize}
  \item
    A level-$i\text{-}1$ grouping connected between a level-$i$ grouping's entry and middle vertices is called the level-$i$ grouping's \emph{A-connection}.
    The edges are called \emph{A-connection edges} (from level $i$ to $i\text{-}1$) and \emph{A-connection return edges} (from level $i\text{-}1$ to level $i$).
  \item
    The level-$i\text{-}1$ groupings connected between a level-$i$ grouping's middle and exit vertices are called \emph{B-connections}.
    The edges are called \emph{B-connection edges} and \emph{B-connection return edges}.
\end{itemize}
Thus, a grouping at level $i \ge 1$ is always connected to groupings at level $i\text{-}1$.
It always has a single A-connection, but can have more than one B-connection.
}

\twrchanged{
Level-0 groupings have no middle vertices.
The edges in a level-$0$ grouping are the decision edges corresponding to the two choices for a decision variable.
}

For $H_2$, the decisions for $x_0$ and $y_0$ are taken in the upper-right (``\emph{fork grouping}'') and lower-right (``\emph{dont-care grouping}'').
\twrchanged{
The red path corresponds to the all-$1$ assignment, which uses the fork grouping twice, as follows:
the $L_1$ grouping's entry vertex;
the connection edge to $L_0$ (solid edge);
decision for $\{ x_0 \mapsto 1 \}$ (right edge);
return edge to the second middle vertex of $L_1$ (solid edge);
connection edge to $L_0$ (dashed edge);
decision for $\{ x_0 \mapsto 1 \}$ (right edge)
return edge to the second exit vertex of $L_1$ (dashed edge);
and edge to the terminal value $\frac{1}{\sqrt{2}}$.
Every grouping can be viewed as a procedure, and the reuse of a grouping  as a procedure call from a different call site.
Note how each ``return'' (solid, dashed) must match the most recent pending ``call'' (solid, dashed, respectively).
All assignments are interpreted with respect to such \emph{matched paths}.
}

\twrchanged{
Whereas a BDD can share sub-DAGs, a procedure call in a CFLOBDD shares the ``middle of a DAG,'' and allows sharing to take place in CFLOBDDs that is not possible in BDDs.
}
\figref{data-structures}(d) shows the CFLOBDD for $H_4$ where the level-$1$ grouping is used 3 times.

Note that variables are not assigned to the decision nodes (``groupings'') in the case of CFLOBDDs.
Because of sharing at all levels, a given decision node does not represent a specific variable,
\twrchanged{
according to the following principle~\cite{DBLP:journals/corr/abs-2302-04349}:
}

\begin{mdframed}[innerleftmargin = 3pt, innerrightmargin = 3pt, skipbelow=-0.0em]
  $\textbf{\CIP}$.
  {\em A level-$0$ grouping is not associated with a specific Boolean variable.
  Instead, the variable that a level-$0$ grouping refers to is determined by context:
  the $n^{\textit{th}}$ level-$0$ grouping visited along a matched path is used to interpret the $n^{\textit{th}}$ Boolean variable.}
\end{mdframed}


==> cflobdd-algos-table.tex <==
\subsection{List of Operations on WCFLOBDDs}
\label{Se:algo-list-cflobdds}

\tableref{algo-list-cflobdds} lists all the operations supported by WCFLOBDDs.
\begin{sidewaystable}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
         \multicolumn{1}{|c|}{\multirow{2}{*}{Operation}} & \multirow{2}{*}{Type Signature} & \multirow{2}{*}{Description} & \multicolumn{2}{|c|}{Time Complexity} \\
         \cline{4-5}
                                                          &                                 &                              &   WCFLOBDD & WBDD \\
         \hline
         \multirow{2}{*}{Equal} & WCFLOBDD $\times$ WCFLOBDD  & \multirow{2}{*}{Checks if two WCFLOBDDs are equal} & \multirow{2}{*}{$\mathcal{O}(1)$} & \multirow{2}{*}{$\mathcal{O}(1)$} \\
         
         & $\rightarrow$ Boolean & & & \\
         \hline
         \multirow{2}{*}{ConstantZero} & \multirow{2}{*}{Int ($k$) $\rightarrow$ WCFLOBDD}  & Creates a WCFLOBDD for & \multirow{2}{*}{$\mathcal{O}(k)$} & \multirow{2}{*}{$\mathcal{O}(1)$} \\
          &  & the function $\lambda x_0 \dots x_{2^k-1}.F$ & & \\
         \hline
         \multirow{2}{*}{ConstantOne} & \multirow{2}{*}{Int ($k$) $\rightarrow$ WCFLOBDD} & Creates a WCFLOBDD for & \multirow{2}{*}{$\mathcal{O}(k)$} & \multirow{2}{*}{$\mathcal{O}(1)$} \\
          &  & the function $\lambda x_0 \dots x_{2^k-1}.T$ & & \\
         \hline
         \multirow{2}{*}{Projection} & \multirow{2}{*}{Int($k$) $\times$ Int($i$) $\rightarrow$ WCFLOBDD} & Creates a WCFLOBDD for & \multirow{2}{*}{$\mathcal{O}(k)$} & \multirow{2}{*}{$\mathcal{O}(2^k)$}\\
         &  & the function $\lambda x_0 \dots x_{2^k-1}. x_i$  & & \\
         \hline
         \multirow{2}{*}{ScalarMultiply} & WCFLOBDD ($c$) $\times$ Value ($v$)  & \multirow{2}{*}{Performs $c' = c \ast v$} & \multirow{2}{*}{$\mathcal{O}(1)$} & \multirow{2}{*}{$\mathcal{O}(1)$} \\
         & $\rightarrow$ WCFLOBDD & & & \\
         \hline
         \multirow{2}{*}{Pointwise Multiplication} & WCFLOBDD ($c_1$) $\times$ WCFLOBDD ($c_2$) & \multirow{2}{*}{Performs $c' = c_1 \,\textit{op}\, c_2$} & \multirow{2}{*}{$\mathcal{O}(|c_1| \times |c_2| \times |c'|)$} & \multirow{2}{*}{$\mathcal{O}(|c_1|_B \times |c_2|_B)$} \\
          &  $\times$ Operation $\textit{op}$ $\rightarrow$ WCFLOBDD &  &  & \\
          \hline
         \multirow{2}{*}{Pointwise Addition} & WCFLOBDD ($c_1$) $\times$ WCFLOBDD ($c_2$) & \multirow{2}{*}{Performs $c' = c_1 \,\textit{op}\, c_2$} & \multirow{2}{*}{$\mathcal{O}(2^{\textit{vars}})$} & \multirow{2}{*}{$\mathcal{O}(2^{\textit{vars}})$} \\
          &  $\times$ Operation $\textit{op}$ $\rightarrow$ WCFLOBDD &  &  & \\
         \hline
         \multirow{2}{*}{PathWeight} & \multirow{2}{*}{WCFLOBDD($c$) $\rightarrow$ WCFLOBDD} & Computes the weight of paths to  & \multirow{2}{*}{$\mathcal{O}(|c|)$}  & \multirow{2}{*}{$\mathcal{O}(|c|_B)$} \\
          &  & every exit vertex of every grouping &  & \\
         \hline
        \multirow{2}{*}{Sampling} & \multirow{2}{*}{WCFLOBDD($c$) $\rightarrow$ String} & \multirow{2}{*}{Samples a path from $c$} & \multirow{2}{*}{$\mathcal{O}(\max (\textit{vars}, |c|))$} & \multirow{2}{*}{$\mathcal{O}(\max (\textit{vars}, |c|_B))$} \\
         &  &  & & \\
         \hline
         \multirow{2}{*}{KroneckerProduct} & WCFLOBDD($c_1$) $\times$ WCFLOBDD($c_2$)  & \multirow{2}{*}{Performs $c' = c_1 \tensor c_2$} & \multirow{2}{*}{$\mathcal{O}(1)$}  & \multirow{2}{*}{$\mathcal{O}(|c_1|_B)$} \\
         & $\rightarrow$ WCFLOBDD & & & \\
         \hline
         \multirow{2}{*}{MatrixMultiply} & WCFLOBDD($c_1$) $\times$ WCFLOBDD($c_2$)  & Performs $c' = c_1 \times c_2$ & $\mathcal{O}(N^3)$, plus the time for & \multirow{2}{*}{$\mathcal{O}(N^3)$} \\
         & $\rightarrow$ WCFLOBDD & for matrices of size $N \times N$ & a final call to \texttt{Reduce} & \\
         \hline
    \end{tabular}
    }
    \caption{
      List of operations on WCFLOBDDs;
      $\textit{vars}$ denotes the number of Boolean variables ($= 2^k$, where $k$ is the number of levels of the WCFLOBDD).
      The size measure $|\cdot|$ counts the number of groupings, vertices, and edges---with no double-counting of shared groupings due to hash-consing.
      In the column for the time complexities of WBDD operations, an occurrence of $c$ refers to a WBDD argument of the operation, and $|c|_B$ denotes the size of WBDD $c$ (the number of nodes and edges).
      Note that the complexity of MatrixMultiply is in terms of the sizes of the matrices represented by $c_1$ and $c_2$, and not the sizes of $c_1$ and $c_2$
      \mas{
      with an added ``final call to Reduce''
      }.
      \mas{
      The algorithm involves a final call to the Reduce procedure. The complexity of Reduce is bounded by the size of the input and output WCFLOBDDs, where the input here refers to the symbolic matrix multiplication (SMM) computation carried out on c1 and c2. The complexity of SMM is O(N^3). Because it is difficult to combine the complexity of SMM and Reduce, we broke out the cost of Reduce as a separate item.
      }
}
    \label{Ta:algo-list-cflobdds}
\end{sidewaystable}

==> eval.tex <==
\section{Evaluation}
\label{Se:eval}

% In this section, we discuss the experiments carried out.
% The experiments are divided into two categories, each answering one of the following questions?

% \twrchanged{
Our experiments were designed to answer two questions:
\begin{itemize}
  \item [\textbf{RQ1:}]
    Can WCFLOBDDs represent substantially larger functions than WBDDs?
  \item [\textbf{RQ2:}]
    In terms of time and space, can WCFLOBDDs outperform WBDDs and CFLOBDDs in a practical domain?
\end{itemize}
% }
We ran all experiments on AWS machines: t2.xlarge machines with 4 vCPUs, 16GB memory, running on Ubuntu OS.

\subsection{Experiments to answer RQ1}
For RQ1, we created five synthetic benchmarks, each defining a family of functions with members having different numbers of variables (all powers of $2$), and tested our implementation of WCFLOBDDs against MQTDD \cite{zulehner2019package} (an implementation of WBDDs):
% The benchmarks were as follows:
\begin{equation*}
  \begin{array}{l@{\hspace{6ex}}l}
    B1: I_n + X_n &     B4: H_n \times I_n + I_n \times X_n \\
    B2: \CNOT_n(0, n-1) \times \CNOT_n(\frac{n}{2}-1, \frac{n}{2}) &     B5: H_n - H_n \\
    B3: H_n \times H_n
  \end{array}
\end{equation*}
where $I_n$, $X_n$, and $H_n$ are the Identity, NOT, and Hadamard matrices, respectively, of size $2^{n/2} \times 2^{n/2}$.
$\CNOT_n(a, b)$ is a Controlled-NOT matrix of size $2^{n/2} \times 2^{n/2}$.
$\CNOT(a, b)(\langle x_0, x_1, \ldots, x_{n/2-1} \rangle) =$
$\langle x_0, \ldots, x_a, \ldots ,(x_a {\oplus} x_b), \ldots, x_{n/2-1} \rangle,~\textrm{for}~x \in \{0,1\}^{n/2}$.

\begin{table}[tb!]
\small{
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Benchmarks} & \multirow{2}{*}{$\log(n)$} & \multicolumn{2}{c|}{WCFLOBDD} & \multicolumn{2}{c|}{MQTDD} \\
    \cline{3-6}
    & & Time (s) & Size & Time (s) & Size \\
    \hline
    \multirow{6}{*}{B1} & 16 & 4.1 & 442 & 13.59 & 65536\\
    & 17 & 16.72 & 470 & 24.94 & 131072\\
    & 18 & 57.33 & 498 & 53.36 & 262144\\
    \cline{5-6}
    & 19 & 241.61 & 526 & \multicolumn{2}{c|}{\multirow{3}{*}{SegFault}}\\
    \cline{3-4}
    & 20 & \multicolumn{2}{c|}{\multirow{2}{*}{Timeout (15min)}} & \multicolumn{2}{c|}{} \\
    & 21 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{}\\
    \hline
    \multirow{6}{*}{B2} & 16 & 0.001 & 654 & 14.56 & 65538\\
    & 17 & 0.001 & 696 & 24.96 & 131074\\
    \cline{5-6}
    & 18 & 0.001 & 738 & \multicolumn{2}{c|}{\multirow{4}{*}{SegFault}}\\
    & 19 & 0.001 & 780 & \multicolumn{2}{c|}{}\\
    & 20 & 0.001 & 822 & \multicolumn{2}{c|}{} \\
    & 21 & 0.001 & 864 & \multicolumn{2}{c|}{}\\
    \hline
    \multirow{6}{*}{B3\tablefootnote{Size for MQTDD is 1 because $H \times H = I$, which is handled as a ``special'' case}} & 16 & 0.001 & 199 & 13.97 & 1\\
    & 17 & 0.001 & 211 & 28.38 & 1\\
    & 18 & 0.001 & 223 & 57.8 & 1\\
    \cline{5-6}
    & 19 & 0.001 & 247 & \multicolumn{2}{c|}{\multirow{3}{*}{SegFault}}\\
    & 20 & 0.001 & 247 & \multicolumn{2}{c|}{} \\
    & 21 & 0.001 & 259 & \multicolumn{2}{c|}{}\\
    \hline
    \multirow{6}{*}{B4} & 16 & \multicolumn{2}{c|}{\multirow{6}{*}{Timeout (15min)}} & 17.9 & 32769\\
    & 17 & \multicolumn{2}{c|}{} & 29.54 & 65537\\
    \cline{5-6}
    & 18 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{\multirow{4}{*}{SegFault}}\\
    & 19 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{}\\
    & 20 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} \\
    & 21 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{}\\
    \hline
    \multirow{6}{*}{B5} & 16 & 0.001 & 83 & 13.97 & 1\\
    & 17 & 0.001 & 88 & 28.54 & 1\\
    & 18 & 0.001 & 93 & 57.48 & 1\\
    \cline{5-6}
    & 19 & 0.001 & 98 & \multicolumn{2}{c|}{\multirow{3}{*}{SegFault}}\\
    & 20 & 0.001 & 103 & \multicolumn{2}{c|}{} \\
    & 21 & 0.001 & 108 & \multicolumn{2}{c|}{}\\
    \hline
    \end{tabular}
    \caption{Execution times and sizes of WCFLOBDDs and WBDDs on synthetic benchmarks}
    \label{Ta:syntheticBenchmarks}
}
\vspace{-5ex}
\end{table}

\tableref{syntheticBenchmarks} shows the performance of WCFLOBDDs and MQTDD (WBDDs) in terms of (i) execution time and (ii) size.
Here ``size'' means the number of vertices and edges for WCFLOBDDs, and the number of nodes for MQTDD.
WCFLOBDDs perform better than MQTDD on all benchmarks except B4, which involves pointwise addition on $H$.
$H$ is a dense matrix, which leads to more Reduce operations on WCFLOBDDs, leading to slower execution time.

\subsection{Experiments to answer RQ2}

\begin{table}[tb!]
    \centering
    {\small
    \setlength{\tabcolsep}{1.5pt}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Circuits} & \multirow{2}{*}{\#Qubits} & \multicolumn{2}{c|}{WCFLOBDD} & \multicolumn{2}{c|}{MQTDD} & \multicolumn{2}{c|}{CFLOBDD} \\
    \cline{3-8}
    & & Time(s) & Size & Time(s) & Size & Time(s) & Size\\
    \hline
    \multirow{5}{*}{\GHZ} & 16 & 0.04 & 138 & 0.01 & 32 & 0.03 & 136\\
    % & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots\\
    & 256 & 0.05 & 250 & 0.13 & 512 & 0.04 & 248 \\
    & 4096 & 0.22 & 362 & 13.33 & 8192 & 0.25 & 360\\
    \cline{5-6}
    & 65536 & 2.4 & 474 & \multicolumn{2}{c|}{\multirow{2}{*}{SegFault}} & 4.6 & 472\\
    & 1048576 & 229.95 & 586 & \multicolumn{2}{c|}{} & 249.4 & 584\\
    \hline
    \multirow{5}{*}{\BV} & 16 & 0.04 & 161 & 0.01 & 18 & 0.05 & 160\\
    & 256 & 0.11 & 716 & 0.2 & 258 & 0.34 & 715 \\
    & 4096 & 1.5 & 5487 & 32.48 & 4098 & 5.58 & 5486\\
    \cline{5-6}
    & 65536 & 44.02 & 58665 & \multicolumn{2}{c|}{\multirow{2}{*}{SegFault}} & 271.6 & 58664\\
    \cline{7-8}
    & 262144 & 438.7 & 218429 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Timeout}\\
    \hline
    \multirow{5}{*}{\textit{DJ}} & 16 & 0.04 & 140 & 0.01 & 18 & 0.05 & 157\\
    & 256 & 0.12 & 244 & 0.24 & 258 & 0.31 & 269 \\
    & 4096 & 1.6 & 348 & 43.9 & 4098 & 5.58 & 381\\
    \cline{5-6}
    & 65536 & 37.5 & 452 & \multicolumn{2}{c|}{\multirow{2}{*}{SegFault}} & 180.4 & 493\\
    \cline{7-8}
    & 262144 & 281.5 & 504 & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Timeout}\\
    \hline
    \multirow{3}{*}{Simon} & 4 & 0.06 & 244 & 0.01 & 33 & 0.05 & 250\\
    & 8 & 0.27 & 1882 & 0.02 & 546 & 0.77 & 2142\\
    \cline{3-4}\cline{7-8}
    & 16 & \multicolumn{2}{c|}{Timeout} & 8.89 & 138798 & \multicolumn{2}{c|}{Timeout}\\
    \hline
    \multirow{4}{*}{Simon\tablefootnote{Reodering of qubits}} & 16 & 0.11 & 243 & 0.02 & 84 & 0.012 & 330\\
    & 256 & 2.5 & 945 & 0.6 & 1525 & 2.92 & 1332\\
    \cline{5-6}
    & 4096 & 208.43 & 7037 & \multicolumn{2}{c|}{\multirow{2}{*}{SegFault}} & 149.94 & 10109\\
    \cline{3-4}
    & 8192 & \multicolumn{2}{c|}{Timeout} & \multicolumn{2}{c|}{} & 455.9 & 17137\\
    \hline
    \multirow{5}{*}{\QFT} & 4 & 0.04 & 61 & 0.01 & 5 & 0.03 & 81\\
    & 16 & 0.05 & 224 & 0.01 & 17 & 182.3 & 22838\\
    \cline{7-8}
    & 256 & 2.17 & 3364 & 2.73 & 257 & \multicolumn{2}{c|}{\multirow{3}{*}{Timeout}}\\
    & 1024 & 37.3 & 13359 & 148.5 & 1025 & \multicolumn{2}{c|}{}\\
    \cline{5-6}
    & 2048 & 205.2 & 26676 & \multicolumn{2}{c|}{Timeout} & \multicolumn{2}{c|}{}\\
    \hline
    \multirow{3}{*}{Grover} & 4 & 0.06 & 110 & 0.01 & 11 & 0.08 & 190\\
    & 8 & 0.28 & 189 & 0.02 & 23 & 28.96 & 1645\\
    \cline{7-8}
    & 16 & 16.17 & 287 & 0.82 & 47 & \multicolumn{2}{c|}{Timeout}\\
    \hline
    \begin{tabular}{@{}c@{}}
     Shor \\
    (15, 2)
    \end{tabular} & 4 & 0.32 & 205 & 0.03 & 26 & \multicolumn{2}{c|}{\multirow{6}{*}{Timeout}}\\
    \cline{1-6}
    \begin{tabular}{@{}c@{}}
    Shor \\
    (21, 2)
    \end{tabular} & 5 & 3.4 & 441 & 0.25 & 84 & \multicolumn{2}{c|}{}\\
    \cline{1-6}
    \begin{tabular}{@{}c@{}}
    Shor \\
    (39, 2)\tablefootnote{Only 39 out of 50 test cases finished before timeout.}
    \end{tabular} & 6 & 190.7 & 3856 & 0.77 & 143 & \multicolumn{2}{c|}{}\\
    \hline
    \end{tabular}
    }

    \caption{Execution times and sizes of WCFLOBDDs, WBDDs, and CFLOBDDs on quantum-circuit benchmarks}
    \label{Ta:quantum-benchmarks}
\end{table}

% \twrchanged{
We applied WBDDs, CFLOBDDs, and WCFLOBDDs to quantum-circuit simulation, which involves exponentially large vectors and matrices.
We used MQTDD \cite{zulehner2019package} and our implementations of CFLOBDDs \cite{Code:CFLOBDDImplementation} and WCFLOBDDs as back ends to Quasimodo~\cite{DBLP:journals/corr/abs-2302-04349}.
We used seven standard quantum circuits:
Greenberger–Horne–Zeilinger state creation (\GHZ), Bernstein–Vazirani algorithm (\BV), Deutsch–Jozsa algorithm (\textit{DJ}), (two versions of) Simon's algorithm\Omit{ (one is a slightly reordered circuit---reordering is done in the placement of the qubits)}, Quantum Fourier Transform (\QFT), Grover's algorithm, and Shor's algorithm.
% }

For each circuit other than \GHZ and \QFT, a ``hidden'' string was initially sampled, and the oracle for the circuit was constructed based on the sampled string.
For \QFT, one of the basis states was sampled and the algorithm changed the basis state into a Fourier-transformed state.
For Shor's algorithm, we used the standard $2n+3$ circuit~\cite{beauregard2002circuit} and report the results for values $(N, a)$, where $N$ is the number to be factored and $a$ is a number used in the phase-estimation procedure.
% \twrchanged{
The following table shows the \emph{circuit width} of each benchmark: the total number of qubits in the circuit as a function of $n$, the number of qubits for, e.g., the hidden string (reported in column 2 of \tableref{quantum-benchmarks}):
% }

\smallskip
\begin{minipage}{0.9\linewidth}
\centering
{\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
     Circuit & \GHZ & \BV & \textit{DJ} & Simon & Grover & Shor \\
    \hline
    Width & $n$ & $n + 1$ & $n + 1$ & $2n$ & $2n-1$ &$2n+3$\\
    \hline
\end{tabular}
}
\end{minipage}

\smallskip
We ran each benchmark 50 times with a 15-minute timeout, starting from a random initial state.
\tableref{quantum-benchmarks} reports average times, and sizes of the final state vector.
For Shor's algorithm (N = 39, a = 2), WCFLOBDDs completed successfully  for only 39 of the 50 runs; the reported results include only those 39 runs.
WCFLOBDDs perform better than MQTDD and CFLOBDDs in most cases. 
The number of qubits that can be handled by WCFLOBDD is 1,048,576 for \GHZ (1$\times$ over CFLOBDDs, 256$\times$ over WBDDs); 262,144 for \BV and \DeutschJozsa (2$\times$ over CFLOBDDs, 64$\times$ over WBDDs); and 2048 for \QFT (128$\times$ over CFLOBDDs, 2$\times$ over WBDDs).
For Simon's algorithm, MQTDD handles up to 16 qubits, whereas WCFLOBDDs and CFLOBDDs only handle 8 qubits.
However, when the qubits are reordered---i.e., $\langle q_0, \ldots, q_{n-1}, q_n, \ldots, q_{2n-1} \rangle$ is changed to $\langle q_0, q_{n}, \ldots, q_{n-1}, q_{2n-1} \rangle$ (with appropriate changes to gate applications)---CFLOBDDs outperform WCFLOBDDs and MQTDD, handling 8192, 4096, and 2048 qubits, respectively.

In cases when WCFLOBDDs, MQTDD, and CFLOBDDs are all successful, the sizes of the final state vector of WCFLOBDDs and CFLOBDDs are similar, and smaller than MQTDD for \GHZ, \BV, \DeutschJozsa, and Simon's algorithm.
% (WCFLOBDDs are slightly better than CFLOBDDs in this case.)
For Grover's algorithm and \QFT, MQTDD represents the final state vector more compactly than WCFLOBDDs and CFLOBDDs.
For \QFT, WCFLOBDDs have substantially better performance than CFLOBDDs.


==> intro.tex <==
\section{Introduction}
\label{Se:intro}

% \twr{
% The Introduction should be similar to my revised abstract, except here we can show the following $2 \times 2$ table, and build the story around what is shown in the table.
% I think you can refer to the four cells as
% (no, no) for BDDs,
% (yes, no) for WBDDs,
% (no, yes) for CFLOBDDs, and
% (yes, yes) for WCFLOBDDs.
% }

%% Context
% Space-efficient representations of data, along with efficient (space and time) operations on the representations are required in many areas of computer science like verification, synthesis, and so on.
% For this purpose, Binary Decision Diagrams (BDDs) are traditionally used in the model-checking community for efficient computations on the data.

Binary Decision Diagrams (BDDs) are a data structure that provides (i) a canonical representation of Boolean functions, relations, matrices, etc., and (ii) algorithms for operating on them in compressed form.
Their introduction was a breakthrough that spurred numerous advances in model checking and equivalence checking for combinational circuits.
%% Gap
%\twrchanged{
% Not all functions have an efficient BDD representation, and 

During the last 45 years, many BDD variants have been introduced to address different failings of vanilla BDDs \cite{DBLP:books/siam/Wegener00}.
One recent innovation is the Context-Free-Language Ordered BDD (CFLOBDD) \cite{DBLP:journals/corr/abs-2211-06818}, a hierarchically structured decision diagram, akin
to BDDs enhanced with a procedure-call mechanism.
This device allows substructures to be shared in ways not possible with BDDs.
For some functions,
CFLOBDDs are exponentially more succinct than BDDs.
Compared with the size of the decision tree for a function, a CFLOBDD---in the best case---can give a double-exponential size reduction.
%}

BDDs were originally designed for Boolean-valued functions, and failed to address the closely related functions: $\{0,1\}^n \rightarrow D$, where $D$ is a set.
Multi-terminal BDDs (MTBDDs) \cite{DBLP:journals/fmsd/FujitaMY97} (or ADDs \cite{DBLP:journals/fmsd/BaharFGHMPS97}) are a relatively straightforward BDD extension for such functions, but have their own drawback: for a function $h$ whose range has a large number of different values $V$ ($V \subseteq D$), the size of an MTBDD (or a multi-terminal CFLOBDD) for $h$ cannot be any smaller than $|V|$.
To date,
the most successful solution to this issue has been \emph{Weighted BDDs} (WBDDs)---BDD-like structures with weights on edges \cite{DBLP:journals/tcad/NiemannWMTD16,DBLP:conf/date/ViamontesMH04}.
For a given assignment $a$ to $h$'s argument variables, $h(a)$ is computed by ``multiplying'' the weights on the path for $a$.
This approach yields succinct representations when factors of the values in $V$ can be reused in the WBDD 
data structure.
% }

\mas
{
Consider two types of functions -- (i) Exponential function $\EXP_n{:}~\{0,1\}^{n} \rightarrow \{2^{j} \mid j \in \{0 \ldots 2^n{-}1\}\}$, where there are $2^n$ unique values and thereby having weights on edges could provide more compression, and (ii) Equality function with $n$ variables $EQ_n : \{0,1\}^{n/2} \times \{0,1\}^{n/2} \rightarrow \{0,1\}$; though the output has only two values, an efficient and more compressed representation is possible by reusing substructures.
}

\mas
{
To represent these two types of functions efficiently, we introduce a new data structure called \emph{Weighted Context-Free-Language Binary Decision Diagrams} (WCFLOBDDs). The data structure borrows ideas from WBDDs, and CFLOBDDs to efficiently represent a broader set of functions than possible heretofore.
}

% This paper combines the CFLOBDD approach with the WBDD approach to 
% \textbf{End Swarst's proposed change}
% 
% %%%%%%%%%%%%%%%%%%%
% 
% \twrchanged{
% Binary Decision Diagrams (BDDs) are used to represent Boolean functions of type $\{0,1\}^n \rightarrow \{0,1\}$ \cite{toc:Bryant86} or
% $\{0,1\}^n \rightarrow D$, where $D$ is a semi-ring \cite{DBLP:journals/fmsd/FujitaMY97,DBLP:journals/fmsd/BaharFGHMPS97}.
% }
% They were a breakthrough data structure for representing Boolean functions, relations, matrices, etc.\ and operating on them in compressed form.
% Their development spurred advances in model checking and equivalence checking for combinational circuits.
% 
% %% Gap
% %\twrchanged{
% % Not all functions have an efficient BDD representation, and 
% During the last 45 years, many BDD variants have been introduced to address different failings of vanilla BDDs \cite{DBLP:books/siam/Wegener00}.
% One recent innovation is a kind of hierarchically structured decision diagram, called Context-Free-Language Ordered BDDs (CFLOBDDs) \cite{DBLP:journals/corr/abs-2211-06818}, which can be thought of as BDDs enhanced with a procedure-call mechanism.
% This device allow substructures to be shared in ways not possible with BDDs.
% Moreover, for some families of functions, CFLOBDDs are exponentially more succinct than BDDs.
% Compared with the size of the decision tree for a function, a CFLOBDD---again, in the best case---can give a double-exponential size reduction.
% %}
% 
% \twrchanged{
% Unfortunately, one failure of (multi-terminal) BDDs \cite{DBLP:journals/fmsd/FujitaMY97} (or ADDs \cite{DBLP:journals/fmsd/BaharFGHMPS97}) also applies to (multi-terminal) CFLOBDDs \cite{DBLP:journals/corr/abs-2211-06818}:
% }
% for a function $h$ whose range has a large number of different values $V$ ($V \subseteq D$), the size of a BDD (or CFLOBDD) for $h$ cannot be any smaller than $|V|$.
% For BDDs, one innovation that addresses this situation is \emph{Weighted BDDs} (WBDDs)---BDD-like structures with weights on edges \cite{DBLP:journals/tcad/NiemannWMTD16,DBLP:conf/date/ViamontesMH04}.
% For a given assignment $a$ to $h$'s argument variables, $h(a)$ is computed by ``multiplying'' the weights on the path for $a$.
% This approach yields succinct representations when factors of the values in $V$ can be reused in the WBDD data structure.
% % }
% 
% %% Innovation
% % \twrchanged{
% This paper combines the two approaches to 
% create \emph{Weighted CFLOBDDs} (WCFLOBDDs).
%Our hope---which turns out to be achievable---was 
We show 
that, in the best case, WCFLOBDDs provide an exponential factor of succinctness over WBDDs and CFLOBDDs.
The following diagram shows the design space of BDDs, WBDDs, CFLOBDDs, and WCFLOBDDs:
\[
  \begin{array}{@{\hspace{0ex}}r@{\hspace{0.95ex}}|r||c@{\hspace{0.65ex}}|@{\hspace{0.65ex}}c@{\hspace{0ex}}}
    \multicolumn{2}{c||}{}                              & \multicolumn{2}{c}{\textrm{Hierarchical}} \\
    \cline{3-4}
    \multicolumn{2}{c||}{}                              & \textrm{no}   & \textrm{yes} \\
    \hline\hline
    \multirow{2}{7ex}{\textrm{Weights}} &  \textrm{no} & \textrm{BDD}~\cite{toc:Bryant86,DBLP:journals/fmsd/FujitaMY97,DBLP:journals/fmsd/BaharFGHMPS97}  & \textrm{CFLOBDD}~\cite{DBLP:journals/corr/abs-2211-06818}  \\
    \cline{2-4}
                                         & \textrm{yes} & \textrm{WBDD}~\cite{DBLP:journals/tcad/NiemannWMTD16,DBLP:conf/date/ViamontesMH04} & \textrm{WCFLOBDD (this paper)} \\
  \end{array}
\]
% }

% Recently, a new data structure for efficient Boolean function representations -- Context-Free-Language Ordered Binary Decision Diagrams (CFLOBDDs) -- has been introduced. CFLOBDDs are a plug-compatible replacement to BDDs and can efficiently represent data in a more compressed fashion compared to BDDs. In the best case, a CFLOBDD for a Boolean function can be smaller than any BDD for that function. CFLOBDDs can be used to represent sets, functions, matrices, etc., efficiently -- a double-exponential compression in the best case -- compared to a decision-tree representation of the same data. CFLOBDDs can provide faster executions and handle problem instances larger than BDDs or decision trees. For this reason, CFLOBDDs are shown to be a good fit for simulations of quantum circuits, where the size of the representation increases exponentially with the number of qubits.

% Consider a function $B_n = \{0,1\}^n \rightarrow D$, where $D$ is a semi-ring. Similar to decision trees and BDDs, the structure of CFLOBDDs has one \emph{``terminal leaf" for every unique value in D}. Naturally, for functions where the number of unique elements in $D$ ($|D|$) increases, the size of CFLOBDDs increases. This is particularly seen in quantum simulations where the probabilities (or amplitudes) may vary for every possible state. For example, a Quantum Fourier Transform (QFT) for $n$ qubits has $2^n$ unique values, leading to $2^n$ unique terminal values in a CFLOBDD, thereby leading to a not-so-efficient representation of QFT using CFLOBDDs (One can observe that even BDDs and decision trees encounter the same issues as that of CFLOBDDs).

% %% Innovation

% To address this issue, we introduce \emph{Weighted Context-Free Language Ordered Binary Decision Diagrams (WCFLOBDDs)}, an extended version of CFLOBDDs that incorporates weights on the edges without compromising the accuracy of function assignments. WCFLOBDDs have at most two terminal values, $0$ and $1$, with the weights spread across the data structure (at level-0 groupings only). The weights are assigned to edges in a WCFLOBDD so that the function is exactly represented, without any loss in accuracy.
% \twrchanged{
% WCFLOBDDs are designed so that the WCFLOBDD for a given function $f$ is a \emph{canonical} representation of $f$.
% }

We evaluated WCFLOBDDs, WBDDs, and CFLOBDDs on both synthetic and quantum-simulation benchmarks, and found that WCFLOBDDs perform better than WBDDs and CFLOBDDs on most benchmarks.
On the quantum-simulation benchmarks, with a 15-minute timeout,
the number of qubits that can be handled by WCFLOBDDs is 1,048,576 for GHZ (1$\times$ over CFLOBDDs, 256$\times$ over WBDDs); 262,144 for BV and DJ (2$\times$ over CFLOBDDs, 64$\times$ over WBDDs); and 2,048 for QFT (128$\times$ over CFLOBDDs, 2$\times$ over WBDDs).
Such results support the conclusion that, at least for some applications, WCFLOBDDs
% provide a much more compressed representation of discrete structures than was previously possible, and 
permit much larger problem instances to be handled than was possible previously.

Our work makes the following contributions:
% \twrchanged{
\begin{itemize}
  \item
    We define WCFLOBDDs, a new data structure to represent Boolean functions, relations, matrices, etc.\ (\sectref{wcflobdds}).
  \item
    We give \emph{algorithms} for WCFLOBDD operations (\sectref{algos}).
  \item
    We show exponential gaps between (i)\,WCFLOBDDs and CFLOBDDs, and (ii)\,WCFLOBDDs and WBDDs 
    (\sectref{separation}).
  \item
    We find that WCFLOBDDs perform as well as or better than WBDDs and CFLOBDDs on most synthetic and quantum-simulation benchmarks (\sectref{eval}).
\end{itemize}
\sectref{back} reviews BDDs, CFLOBDDs, and WBDDs.
% }
\sectref{related} discusses related work.
% \sectref{conclusion} concludes.

==> pair-product.tex <==
\subsection{Pointwise Multiplication}
\label{Se:pointwise-mult}

% \twrnew{
The pseudocode for the algorithm for pointwise multiplication of WCFLOBDDs
% }
is shown in~\algref{MBO}, which calls~\algref{PairProduct} and~\algref{Reduce} , which in turn call~\algrefs{InducedTuples}{InsertBConnection}.
\begin{itemize}
  \item
    \algref{PairProduct} recursively performs the cross-product of input groupings $g1$, $g2$ to form a new grouping $g$, along with $pt$, which is a tuple of exit-vertex pairs.
  \item
    \algref{InducedTuples} collapses $pt$ to enforce structural invariants on the value tuple.
  \item
% \twrchanged{
    \algref{Reduce} reduces a grouping based on return tuples or the value tuple, and as a by-product ensures canonicity of the resulting WCFLOBDD (see  \sectref{AlgorithmsUsedInPointwiseMultiplication}).
% }
  \item
% \twrchanged{
    \algref{InsertBConnection} determines the position for a B-connection in a grouping being constructed, reusing one if it is already present in the grouping (see  \sectref{AlgorithmsUsedInPointwiseMultiplication}).
% }
\end{itemize}

\begin{algorithm}[tb!]
\caption{Pointwise Multiplication\label{Fi:MBO}}
\small{
\Input{WCFLOBDDs n1 = $\langle \textit{fw1}, g1, \textit{vt1} \rangle$, n2 = $\langle \textit{fw2}, g2, \textit{vt2} \rangle$}
\Output{CFLOBDD n = n1 $\cdot$ n2}
\Begin{
\tcp{Perform cross product}
    Grouping$\times$PairTuple [g,pt] = PairProduct(g1,g2)\;  \label{Li:BAAR:CallPairProduct}
    ValueTuple deducedValueTuple = [ vt1[i1] $\cdot$ vt2[i2]~:~[i1,i2] $\in$ pt ]\;  \label{Li:BAAR:LeafValues}
     \tcp{Collapse duplicate leaf values, folding to the left}
    Tuple$\times$Tuple [inducedValueTuple,inducedReductionTuple] = CollapseClassesLeftmost(deducedValueTuple)\;  \label{Li:BAAR:CollapseLeafValues}
    Grouping$\times$Weight [g', $\textit{fw}$] = Reduce(g, inducedReductionTuple, deducedValueTuple)\;  \label{Li:BAAR:CallReduce}
    WCFLOBDD n = RepresentativeCFLOBDD($\textit{fw} \cdot \textit{fw1} \cdot \textit{fw2}$, g', inducedValueTuple)\;
    \Return n\;
}
}
\end{algorithm}

\begin{algorithm}[tb!]
\caption{PairProduct\label{Fi:PairProduct}}
\small{
\Input{Groupings g1, g2}
\Output{Grouping g: product of g1 and g2; PairTuple ptAns: tuple of pairs of exit vertices}
\SetKwBlock{Begin}{Begin}{}
\Begin{
    \lIf {g1 and g2 are both ConstantOneProtoCFLOBDD \label{Li:PPConstantOneStart}}  
    { \Return [ g1, [[1,1]] ]}   
    \lIf {g1 or g2 is ConstantZeroProtoCFLOBDD }  
    { \Return [ ConstantZeroProtoCFLOBDD(g1.level), [[1,1]] ]}   
    \lIf {g1 is ConstantOneProtoCFLOBDD}
    {\Return [ g2, [[1,k]~:~k $\in$ [1..g2.numberOfExits]] ]}
    \lIf {g2 is ConstantOneProtoCFLOBDD}
    {\Return [ g1, [[k,1]~:~k $\in$ [1..g1.numberOfExits]] ]}      \label{Li:PPConstantOneEnd}
\tcp{Similar cases for other base cases, with appropriate pairings of exit vertices}
\If {g1 and g2 are fork groupings  \label{Li:PPBothForkGroupings}} {
    ForkGrouping g = new ForkGrouping(g1.lw $\cdot$ g2.lw, g1.rw $\cdot$ g2.rw)\;
\Return [ g, [[1,1],[2,2]] ]\;
} \label{Li:PPBothForkGroupingsEnd}
\tcp{ Pair the A-connections}
    Grouping$\times$PairTuple [gA,ptA] = PairProduct(g1.AConnection, g2.AConnection)\;
    InternalGrouping g = new InternalGrouping(g1.level)\;
    g.AConnection = gA\;
    g.AReturnTuple = [1..$|$ptA$|$]\tcp*[r]{Represents the middle vertices}
    g.numberOfBConnections = $|$ptA$|$\;  \label{Li:PPNumberOfBConnections}
    \tcp{Continued in \algref{PairProductContinued}}
}
}
\end{algorithm}

\begin{algorithm}[tb!]
%% \SetAlgoRefName{\ref{Fi:PairProduct}}   %% Introduces error
\caption{PairProduct (cont.)\label{Fi:PairProductContinued}}
\setcounter{AlgoLine}{13}
\SetKwBlock{Begin}{}{end}
\small{
\Begin{
    \tcp{Pair the B-connections, but only for pairs in ptA }
    \tcp{Descriptor of pairings of exit vertices}
    Tuple ptAns = []\;  \label{Li:ptAnsDeclaration}

    \tcp{Create a B-connection for each middle vertex}
    \For {$j \leftarrow 1$ \KwTo $|ptA|$}{
        Grouping$\times$PairTuple [gB,ptB] = PairProduct(g1.BConnections[ptA(j)(1)], g2.BConnections[ptA(j)(2)])\;
        g.BConnections[j] = gB \;
        \tcp{Create g.BReturnTuples[j], and augment ptAns as necessary}
        g.BReturnTuples[j] = [] \;        \label{Li:PPExitVertexLoopStart}
        \For{$i \leftarrow 1$ \KwTo $|ptB|$} {
            c1 = g1.BReturnTuples[ptA(j)(1)](ptB(i)(1))\tcp*[r]{a g1 exit}
            c2 = g2.BReturnTuples[ptA(j)(2)](ptB(i)(2)) \tcp*[r]{a g2 exit}
            \eIf(\tcp*[f]{Not a new exit vertex of g}){[c1,c2] $\in$ ptAns}
                {
                index = the k such that ptAns(k) == [c1,c2] \;
                g.BReturnTuples[j] = g.BReturnTuples[j] $||$ index \;
                }
            (\tcp*[f]{Identified a new exit vertex of g}){
                g.numberOfExits = g.numberOfExits + 1 \;
                g.BReturnTuples[j] = g.BReturnTuples[j] $||$ g.numberOfExits \;
                ptAns = ptAns $||$ [c1,c2] \; \label{Li:PPConcatenateExitPair}
            }
        }  \label{Li:PPExitVertexLoopEnd}
    }
    \Return [RepresentativeGrouping(g), ptAns]\; \label{Li:PPTabulateAnswer}
}
}
\end{algorithm}


\begin{algorithm}[tb!]
\caption{CollapseClassesLeftmost\label{Fi:InducedTuples}}
\small{
\Input{Tuple equivClasses}
\Output{Tuple$\times$Tuple [projectedClasses, renumberedClasses]}
\Begin{
\tcp{Project the tuple equivClasses, preserving left-to-right order, retaining the leftmost instance of each class}
\label{Li:IT:TupleCollapseStart}
Tuple projectedClasses = [equivClasses(i) : i $\in$ [1..$|$equivClasses$|$] $|$ i = min\{j $\in$ [1..$|$equivClasses$|$] $|$ equivClasses(j) = equivClasses(i)\}]\;
\label{Li:IT:TupleCollapseEnd}
\tcp{Create tuple in which classes in equivClasses are renumbered according to their ordinal position in projectedClasses}
Map orderOfProjectedClasses = \{[x,i]: i $\in$ [1..$|$projectedClasses$|$] $|$ x = projectedClasses(i)\}\;
Tuple renumberedClasses = [orderOfProjectedClasses(v) : v $\in$ equivClasses]\;
\Return [projectedClasses, renumberedClasses]\;
}
}
\end{algorithm}

==> performance-plots.tex <==
\subsection{Experimental Results}

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/ghz_time_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/bv_time_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/dj_time_new.pdf}
    \end{subfigure}
    \caption{Performance of WCFLOBDDs, MQTDD, and CFLOBDDs on various quantum benchmarks with an increasing number of qubits. The vertical axis indicates the time in seconds
    and the horizontal axis indicates $\log$ \#Qubits.}
    \label{Fi:results_time}
\end{figure}

\begin{figure}[tb!]
    \ContinuedFloat
    \centering
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/simons_time_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/simons2_time_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/qft_time_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/grovers_time_new.pdf}
    \end{subfigure}
    \caption{(Continued.)}
\end{figure}

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/ghz_size_new.pdf}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/bv_size_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/dj_size_new.pdf}
    \end{subfigure}
    \caption{Performance of WCFLOBDDs, MQTDD, and CFLOBDDs on various quantum benchmarks with an increasing number of qubits. The vertical axis indicates the size
    and the horizontal axis indicates $\log$ \#Qubits.}
    \label{Fi:results_size}
\end{figure}

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/simons_size_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/simons2_size_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/qft_size_new.pdf}
    \end{subfigure}
    \begin{subfigure}{0.85\columnwidth}
    \includegraphics[width=\linewidth]{figures/grovers_size_new.pdf}
    \end{subfigure}
    \caption{(Contind.)}
\end{figure}

\figrefs{results_time}{results_size} compare the performance of WCFLOBDDs, MQTDD, and CFLOBDDs on quantum-circuit-simulation benchmarks, in terms of execution time and size, respectively.

==> separation-proofs.tex <==
\subsection{Proof of Separation Between WCFLOBDDs and WBDDs}
\label{Se:SeparationProofVersusWBDDs}

\noindent
{\bf Theorem~\ref{The:HadamardSeparation}.}
The Hadamard relation $H_n:\{0,1\}^{n/2} \times \{0,1\}^{n/2} \rightarrow \{1,-1\}$ between variable sets ($x_0\cdots x_{n/2-1}$) and ($y_0\cdots y_{n/2-1}$), defined as $H_n = H_{n/2} \otimes H_{n/2}$,
$H_2 = H = \frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
        1 & 1\\
        1 & -1
    \end{smallmatrix}\right]$,
where $n = 2^l$ and $\otimes$ denotes Kronecker product, can be represented by a WCFLOBDD with $\bigO(\log{n})$ vertices and edges.
A WBDD for $H_n$ requires $\bigOmega(n)$ nodes.

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.8\linewidth}
%         \includegraphics[width=\linewidth]{figures/walsh2_wcflobdd.pdf}
%         \caption{WCFLOBDD for $H_4$}
%     \end{subfigure}
%     \vspace{2.0ex}
%     \begin{subfigure}{0.52\linewidth}
%         \includegraphics[width=\linewidth]{figures/walshn_wcflobdd.pdf}
%         \caption{WCFLOBDD for $H_n$ (topmost level only)}
%     \end{subfigure}
%     \caption{WCFLOBDD Representation for $H_n$.}
%     \label{Fi:wcflobdd_walsh}
% \end{figure}

\begin{proof}
\,\newline
\textit{WCFLOBDD Claim.} \figref{wcflobdd_hadamard}(a) shows the WCFLOBDD representation for the base case of $n = 2, H_2$.~\figref{wcflobdd_hadamard}(b), and~\figref{wcflobdd_hadamard}(c) show the WCFLOBDD representation for the next two function in this series, $n = 2, H_4 = H_2 \otimes H_2$, and $n = 3, H_8 = H_4 \tensor H_4$.
The level-2 grouping of $H_4$ is connected to the level-1 grouping (which represents $H_2$) through both its A-connection and B-connection.
The A-connection corresponds to the left-most $H_2$ of $H_2 \otimes H_2$ and the B-connection corresponds to the right-most $H_2$ of $H_2 \otimes H_2$.
Let $P(l)$ denote the number of vertices, edges, and groupings at level-$l$, then $P(1) = 30$, and $P(2) = P(1) + 8 = 38$.\footnote{
  Note that $P(1)$ contributes just once because every grouping has only one representative in memory.
}
Generalizing to arbitrary $l = \log n$, as shown by \figref{wcflobdd_hadamard}(d), the recurrence equation for $P(l)$ is $P(l) = P(l-1) + 8$, which has the solution $P(l) = 8*l + 22$.
Consequently, $H_n$ can be represented by a WCFLOBDD that has only $\bigO(\log n)$ vertices and edges.
\,\newline
\textit{WBDD Claim.}
We claim that regardless of the variable ordering, a WBDD that represents $H_n$ requires at least $n$ nodes---one node for each argument variable.
We prove this claim by contradiction.
Suppose that there exists a WBDD $B$ that represents $H_n$, but does not have at least one node for every argument variable (call the variable $z$, speaking generically).
We will establish a contradiction by showing that the function $B_n$ that $B$ actually represents does not depend on $z$.

Consider the all-true assignment: $\mathcal{T} \eqdef \forall k \in \{0..n/2-1 \}, x_k \mapsto T, y_k \mapsto T$. There are three possible cases:
\begin{itemize}
    \item Case 1: Consider the case where $B$ does not depend on variable $y_k$, for some $k \in \{0...n/2-1 \}$. Consider two variable assignments $A_1 \eqdef \mathcal{T}$ and $A_2 \eqdef \mathcal{T}[y_k \mapsto F]$ (i.e., $A_2$ is $A_1$ with $y_k$ updated to $F$). $A_1$ and $A_2$ yield the same value for the function represented by $B$,
    but they yield different values for the Hadamard relation.
    That is, if $H_n[A_1] = v$ 
    (where $v$ is either $\frac{1}{\sqrt{2^{n/2}}}$ or $\frac{-1}{\sqrt{2^{n/2}}}$),
    then $H_n[A_2] = -v$.
    We prove this claim by induction on the ``level'' (i.e., the $\log$ of the number of Boolean variables).
    \begin{proof}
    
    \smallskip
    \noindent
    Base Case: 
    \begin{itemize}
        \item $n = 2$. $H_2[A_1]$ is the value of the path $[x_0 \mapsto T, y_0 \mapsto T]$, the lower-right corner of $H_2$, which is $\frac{-1}{\sqrt{2}}$, and
        $H_2[A_2]$ is the value of the path $[x_0 \mapsto T, y_0 \mapsto F]$, which yields $\frac{1}{\sqrt{2}}$.
        \item $n = 4$. $A_1$ is again the path to the lower-right corner of $H_4$, which yields a value of $\frac{1}{2}$. For $A_2$, the path depends on the value of $k$.
        For $k = 0$, $A_2$ gives the value of row $4$ and column $2$ of $H_4$,
        which is $-\frac{1}{2}$; if $k = 1$, $A_2$ ends up at row $4$ and column $3$, which is also $-\frac{1}{2}$.
    \end{itemize}
    Induction Step: To prove this claim for any level, let us extend the notation for $A_1$ and $A_2$ by adding level information.
    Let $A_1^m$ denotes the ``all-true'' assignment for $2^m$ variables, and $A_2^m = A_1^m[y_k \mapsto F]$ is $A_1$ with $y_k$ updated to $F$.
    Let us assume that the claim is true for $H_{2^m}$, i.e.,
    $H_{2^m}[A_1^{m}] = v$ (which could be $\frac{1}{\sqrt{2^{m/2}}}$ or $\frac{-1}{\sqrt{2^{m/2}}}$) and $H_{2^m}[A_2^{m}] = -v$.
    We must show that the claim holds true for $H_{2^{m+1}}$.

    We know that $H_{2^{m+1}} = H_{2^m} \tensor H_{2^m}$.
    Thus,
    $H_{2^{m+1}}[A_1^{m+1}] = H_{2^m}[A_1^{m}] \ast H_{2^m}[A_1^{m}] = v \ast v  = v^2$,
    where $A_1^{m + 1} = A_1^m || A_1^m$.
    Similarly, we can write a recursive relation for assignment $A_2^{m+1}$,
    depending on the position of the bit-flip for $y$. There are two possible cases:
    \begin{enumerate}
      \item
        $k$ occurs in the first half; $A_2^{m + 1} = A_2^m || A_1^m$ and therefore, 
        $H_{2^{m+1}}[A_2^{m+1}] = H_{2^m}[A_2^{m}] \ast H_{2^m}[A_1^{m}]$,
        which, by induction, leads to a value of $-v \ast v = -v^2$.
      \item
        $k$ occurs in the second half; $A_2^{m + 1} = A_1^m || A_2^m$ and therefore, 
        $H_{2^{m+1}}[A_2^{m+1}] = H_{2^m}[A_1^{m}] \ast H_{2^m}[A_2^{m}]$,
        which, by induction, leads to a value of $v \ast -v = -v^2$.
    \end{enumerate}
    In both cases, the values obtained with $y_k$ updated to $F$ (bit-flip) do not match the value
    for the all-true assignment $\mathcal{T}$.
    \end{proof}
    We conclude that none of the $y_k$ variables can be dropped individually.

  \item
    Case 2:
    Using a completely analogous argument to Case 1, none of the $x_k$ variables can be dropped individually.
  \item
    Case 3: $B$ does not depend on either $x_k$ or $y_k$.
    The assignments
    $A_1 = \mathcal{T} = [...,{x_k}\mapsto T, {y_k}\mapsto T,...]$, 
    $A_2 = \mathcal{T}[y_k \mapsto F] = [...,{x_k}\mapsto T, {y_k}\mapsto F,...]$, 
    $A_3 = \mathcal{T}[x_k \mapsto F] = [...,{x_k}\mapsto F, {y_k}\mapsto T,...]$ and 
    $A_4 = \mathcal{T}[x_k \mapsto F, y_k \mapsto F] = [...,{x_k}\mapsto F, {y_k}\mapsto F,...]$ must all be mapped to the same value by the function represented by $B$, which violates the definition of the Hadamard relation $H_n$.
    (More precisely, $H_n[A_1] = v^2$, where $v$ is either $\frac{1}{\sqrt{2^{n/2}}}$ or $\frac{-1}{\sqrt{2^{n/2}}}$, but $H_n[A_2] = H_n[A_3] = H_n[A_4] = -v^2$, which can be proved using an inductive argument similar to Case 1.)
    Consequently, $(x_k, y_k)$ cannot be dropped as a pair.
\end{itemize}
\end{proof}


\subsection{Proof of Separation Between WCFLOBDDs and CFLOBDDs}
\label{Se:SeparationProofVersusCFLOBDDs}

\noindent
{\bf Theorem~\ref{The:NumberSeparation}.}
For $n = 2^l$, where $l \geq 0$,
$\EXP_n$,
defined over the variables $\{x_0\cdots x_{n-1}\}$, 
can be represented by a WCFLOBDD with $\bigO(n)$ vertices and edges.
A CFLOBDD
that uses only the variables $\{x_0\cdots x_{n-1}\}$
for $\EXP_n$ requires $\bigOmega(2^n)$ vertices and edges.

\begin{proof}
\,\newline
\textit{CFLOBDD Claim.} 
Only the $n$ variables ($x_0 \dots x_{n-1}$) can be used in the CFLOBDD that represents \EXP$_n$; no additional variables are allowed.
The relation $\EXP_n$ has $2^n$ unique elements.
A CFLOBDD that represents $\EXP_n$ will have $2^n$ terminal values; hence, the CFLOBDD that represents this relation will have at least $\Omega(2^n)$ vertices and edges.
\,\newline
\textit{WCFLOBDD Claim.} Consider the WCFLOBDD $C$ with variable ordering $\langle x_{n-1}, \cdots, x_0 \rangle$, where $C$ contains $n$
level-$0$ groupings corresponding to the $n$ decision variables in $\EXP_n$.
Let the level-$0$ grouping for variable $x_i$
have the weights $(1, 2^i)$.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.15\linewidth}
    \includegraphics[width=0.8\linewidth]{figures/num_1.pdf}
    \caption{WCFLOBDD for $\EXP_1$}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.35\linewidth}
    \includegraphics[width=0.8\linewidth]{figures/num_2.pdf}
    \caption{WCFLOBDD for $\EXP_2$}
    \end{subfigure}
    \begin{subfigure}{0.37\linewidth}
    \includegraphics[width=0.8\linewidth]{figures/num_4.pdf}
    \caption{WCFLOBDD for $\EXP_n$ (topmost level only)}
    \end{subfigure}
    \caption{WCFLOBDD representation for \EXP$_n$.}
    \label{Fi:num_rel}
\end{figure}

The construction of the WCFLOBDD representation of $\EXP_n$ is depicted in~\figref{num_rel}.
Let $P(l)$ denote the number of vertices, edges, and groupings
for \EXP$_n$ for $n$ variables and $l$ levels, where $n = 2^l$.
\figref{num_rel}(a) shows the WCFLOBDD representation for $\EXP_1$ with one variable $x_0$, so $P(0) = 6$.
\figref{num_rel}(b) shows the WCFLOBDD representation for \EXP$_2$ with two variables $x_1, x_0$.
We see that the WCFLOBDD for $\EXP_2$ has one level-1 grouping with ``calls" to two different ``level-0" groupings for $x_1, x_0$. 
In this case, $P(1) = 9 + (P(0) - 1) + (P(0) - 1) = 2P(0) + 7 = 19$.
Extending this to the case of $n$ variables, we find that $P(l) = 2(P(l-1) - 1) + 9$ (as shown in~\figref{num_rel}(c)). Solving this recurrence equation, we get $P(l) = 13 * 2^l - 7 = \bigO(2^l) = \bigO(n)$.

Hence, $\EXP_n$ can be represented by a WCFLOBDD that has $\bigO(n)$ vertices and edges.
\end{proof}




==> separation.tex <==
\section{Exponential Succinctness Gaps}
\label{Se:separation}

% \twrchanged{
We established exponential gaps between (i) WCFLOBDDs and CFLOBDDs, and (ii) WCFLOBDDs and WBDDs. 
\mas{
See Proofs in Appendices \sectref{SeparationProofVersusCFLOBDDs} and \sectref{SeparationProofVersusWBDDs}
}
% }

\begin{definition}
\label{De:NumberRelation}
The $n$-bit exponential function $\EXP_n{:}~\{0,1\}^{n} \rightarrow \{2^{j} \mid j \in \{0 \ldots 2^n{-}1\}\}$ on variables ($x_0\cdots x_{n-1}$) is
\[
  \EXP_n(X) \eqdef \Pi_{i=0}^{n-1} 2^{2^i * x_i}
              =    2^{\sum_{i=0}^{n-1} {2^i * x_i}}
              =    2^{\textit{BinaryValue}(X)}
\]
\end{definition}

\begin{theorem}\label{The:NumberSeparation}
For $n = 2^l$, where $l \geq 0$,
$\EXP_n$ can be represented by a WCFLOBDD with $\bigO(n)$ vertices and edges.
A CFLOBDD for $\EXP_n$ requires $\bigOmega(2^n)$ vertices and edges.
\end{theorem}

% \begin{proof}
% See Appendix \sectref{SeparationProofVersusCFLOBDDs}
% \end{proof}

\begin{theorem}\label{The:HadamardSeparation}
The Hadamard relation $H_n:\{0,1\}^{n/2} \times \{0,1\}^{n/2} \rightarrow \{1,-1\}$ between variable sets ($x_0\cdots x_{n/2-1}$) and ($y_0\cdots y_{n/2-1}$), defined as $H_n = H_{n/2} \otimes H_{n/2}$,
$H_2 = H = \frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
        1 & 1\\
        1 & -1
    \end{smallmatrix}\right]$,
where $n = 2^l$ and $\otimes$ denotes Kronecker product, can be represented by a WCFLOBDD with $\bigO(\log{n})$ vertices and edges.
A WBDD for $H_n$ requires $\bigOmega(n)$ nodes.
\end{theorem}

% \begin{proof}
% See Appendix \sectref{SeparationProofVersusWBDDs}
% \end{proof}


==> wcflobdds.tex <==
\section{Weighted CFLOBDDs (WCFLOBDDs)}
\label{Se:wcflobdds}

\subsection{Weights and the Basic Structure of WCFLOBDDs}

\begin{figure}
  \centering
  % \begin{subfigure}{0.3\linewidth}
  \includegraphics[width=0.45\linewidth]{figures/walsh1_wcflobdd-cropped.pdf}
  % \end{subfigure}
  % \begin{subfigure}{0.33\linewidth}
  % \includegraphics[width=0.9\linewidth]{figures/walsh2_wcflobdd.pdf}
  % \end{subfigure}
  % \begin{subfigure}{0.33\linewidth}
  % \includegraphics[width=0.9\linewidth]{figures/walshn_wcflobdd.pdf}
  % \end{subfigure}
  \caption{
    WCFLOBDD for the Hadamard matrix $\frac{1}{\sqrt{2}}\left[\begin{smallmatrix}
      1 & 1\\
      1 & -1
  \end{smallmatrix}\right]$,
  with the variable ordering $\langle x_0, y_0 \rangle$ ($x_0$: row; $y_0$: column).
  }
  \label{Fi:wcflobdd_hadamard}
  \vspace{-3ex}
\end{figure}

\begin{definition}
Let $\mathcal{D} = \langle A, +, \cdot, \bar{0}, \bar{1} \rangle$ be a set with two binary operations $+$ and $\cdot$.
$\mathcal{D}$ is called a \textbf{semi-field} if, for all $a, b, c \in \mathcal{D}$, the following properties are satisfied:
\begin{equation*}
  \begin{array}{l@{\hspace{2.5ex}}r@{\hspace{0.75ex}}c@{\hspace{0.75ex}}l}
    \textrm{Associativity:}  & a + (b + c) & = & (a + b) + c \\
                             & a \cdot (b \cdot c) & = & (a \cdot b) \cdot c \\
    \textrm{Commutativity:}  & a + b & = & b + a \\
    \textrm{Identity:}       & \multicolumn{3}{l}{
                                 a + \bar{0} = a \qquad\quad
                                 a \cdot \bar{1} = a
                             } \\
    \textrm{Annihilation:}   & a \cdot \bar{0} & = & \bar{0} \\
    \textrm{Distributivity:} & a \cdot (b + c) & = & (a \cdot b) + (a \cdot c) \\
    \textrm{Multiplicative Inverse:} & \multicolumn{3}{c}{a \neq 0 \Rightarrow \exists a^{-1} \in \mathcal{D} : a^{-1} \cdot a = \bar{1}}
  \end{array}
\end{equation*}
\end{definition}
% \twrchanged{
A semi-field has no zero divisors:
$a \neq 0 \land a \cdot b = 0$ $\Rightarrow$ $a^{-1} \cdot a \cdot b = 0$ $\Rightarrow$ $b = 0$.
% }

WCFLOBDDs can be viewed as \emph{single-entry, multi-exit, weighted hierarchical systems}.
They are similar to CFLOBDDs except that instead of different terminal values, edges of level-$0$ groupings are labeled with semi-field \emph{weights};
their product gives the value of a (matched) path.
\figref{wcflobdd_hadamard} shows the WCFLOBDD representation of Hadamard matrix $H$. 
% WCFLOBDDs and CFLOBDDs have somewhat similar structures.
% \twrchanged{
The main structural elements of a WCFLOBDD are as follows:
% }
\begin{itemize}
  \item
% \twrchanged{
    A WCFLOBDD has a hierarchical structure.
% }
    Every oval-shaped structure is called a \emph{grouping} and every grouping is associated with a level. In~\figref{wcflobdd_hadamard}, there are 4 groupings, of which three are at level 0 and one is at level 1.
  \item
    The vertex (dot) at the top of each grouping is called an \emph{entry vertex}, the vertices in the middle of a grouping are \emph{middle vertices}, and the vertices at the bottom of the grouping are \emph{exit vertices}.
    Level-0 groupings have no middle vertices.
    The three sets of vertices are disjoint.
  \item
    The groupings connected between entry and middle vertices called \emph{A-Connections};
    the edges are called \emph{A-Connection edges} (from level $i$ to $i-1$) and \emph{A-Connection return edges} (from level $i-1$ to level $i$).
  \item
    The groupings between middle and exit vertices are called \emph{B-Connections};
    the edges are called \emph{B-Connection edges} and \emph{B-Connection return edges}.
  \item
    A grouping at level $i \ge 1$ is always connected to groupings at level $i-1$.
    It always has a single A-Connection, but can have more than one B-Connection.
  \item
% \twrchanged{
    The incoming edge to the entry-vertex of the topmost-level
% }
    grouping is called a \emph{free-edge}.
  \item
    There are additional structural properties for weights:
    \begin{itemize}
      \item
        Every level-0 grouping~\footnote{\mas{Only the level-0 grouping edges are assigned semi-field weights and no other edges are assigned weights to ensure canonicity. Adding weights to edges at level-k groupings leads to canonicity issues.}} has a pair of weights $(lw, rw)$, $lw, rw \in \mathcal{D}$, where $\mathcal{D}$ is a semi-field. $lw$ is the weight for the decision-edge for $0$ (false);
        $rw$ is the weight for the decision-edge for $1$ (true).
      \item
        The weight $f \in \mathcal{D}$ associated with the free edge is called the \emph{factor weight}.
      \item
        The terminal values connected to the exit vertices of the top-level grouping can only be $\bar{0}, \bar{1} \in \mathcal{D}$.
    \end{itemize}
    % \begin{itemize}
    %     \item The edges at level-0 groupings (the decision groupings) are associated with weights. The weight associated with the left edge (corresponding to decision $F$) is called $lweight$ and the right edge (corresponding to decision $T$) is called $rweight$. The type of the weights will be the type of the domain of the function being represented. In case of~\figref{wcflobdd_hadamard}, the weights are of type ${\tt double}$.
    %     \item The exit vertices of the top-level grouping are connected to at most two terminal values - \emph{AnnhilatorValue} and \emph{IdentityValue}. In cases where ${\tt double}$~\footnote{same for ${\tt int, complex}$, etc.} is the weight type, the \emph{AnnhilatorValue} would be 0 and \emph{IdentityValue} would be 1.
    %     \item The free-edge connected to the top-level grouping is called \emph{factor-edge} and is associated with a weight.
    %     \item Every other (non-decision-related) edge has weight of \emph{IdentityValue}. In the case of ${\tt double}$ weight type, the edge has the weight of $1$. This weight is implicit and never explicitly recorded.
    % \end{itemize}
\end{itemize}
% \twrchanged{
Formally, a WCFLOBDD is a triple $\langle f, G, V \rangle$, where $f \in \mathcal{D}$ is the factor weight of the free-edge, $G$ is a grouping, and $V \in \{ [\bar{0}], [\bar{1}], [\bar{0}, \bar{1}], [\bar{1}, \bar{0}] \}$ \mas{(where, [] indicates a tuple)} is the sequence of terminal values.
% }

We describe the range of $V$ in detail:
\begin{itemize}
    \item $[\bar{0}]$ only occurs for the function lambda $\vec{x}. 0$. All leaves of the decision tree are $\bar{0}$.
    \item $[\bar{1}]$ occurs for a function for which the value is never $\bar{0}$ (for any assignment to the Boolean variables). No leaf of the decision tree is $\bar{0}$.
    \item  $[\bar{1}, \bar{0}]$ occurs when a function has the value $\bar{0}$ for some assignment, but not for the all-0 assignment (i.e., in the decision tree, the all-0 assignment runs down the left side of the tree to the leftmost leaf; that leaf is not $0$ in the decision tree)
    \item  $[\bar{0}, \bar{1}]$ occurs when a function has the value $\bar{0}$ for the all-0 assignment (and possibly other assignments, but at least one assignment does not yield $\bar{0}$). In other words, the leftmost leaf of the decision tree is $\bar{0}$.

\end{itemize}

\emph{Function evaluation.}
% \twrchanged{
Given WCFLOBDD $C$ that represents $h: \{0,1\}^n \rightarrow \mathcal{D}$ and an assignment $a$ for $h$'s arguments,
the value $h(a)$ is obtained from $C$, denoted by $\sem{C}(a)$, as the product of the edge weights on the path for $a$ in $C$.
Formally,
\[
    \sem{C}(a) \eqdef f \cdot \sem{G}(a) \cdot V[i].
\]
Here $i = \langle G \rangle(a)$, where $\langle G \rangle (a)$ returns the exit-vertex index of $G$ reached by following the path for assignment $a$, and
\[
  \sem{G}(a) \eqdef \sem{G.\AConnection}(a_1) \cdot \sem{G.\BConnection[j]}(a_2),
\]
where $j = \langle G.\AConnection \rangle (a_1)$, and  $a_1 || a_2 = a$.
% }

In the case of~\figref{wcflobdd_hadamard},
% \twrchanged{
$\mathcal{D} = \langle \mathbb{R}, +, \times, 0, 1 \rangle$.
% }
For $a = \{ x_0 \mapsto 1, y_0 \mapsto 1 \}$, the path highlighted in bold in~\figref{wcflobdd_hadamard} evaluates to $H[1][1] = \frac{1}{\sqrt{2}} \times 1 \times -1 \times 1 = \frac{-1}{\sqrt{2}}$.

\subsection{Canonicity}
\label{Se:canonicity}

As with other decision diagrams, we can ensure \emph{canonicity}---that every function has a unique representation---by imposing certain structural invariants \cite[p.\ 48]{DBLP:books/siam/Wegener00}, \cite[\S4.1]{DBLP:journals/corr/abs-2211-06818}.

\begin{definition}\label{De:StructuralInvariants}
% \twrchanged{
    A \emph{\protoWCFLOBDD} at level $k$ is a hierarchical structure made up of some number of \emph{groupings}---of which there is one grouping at level $k$, and at least one at each level $0, \ldots, k{\textrm{--}}1$---that satisfies the \emph{structural invariants} given below.
    (See also \cite[Fig.\ 8]{DBLP:journals/corr/abs-2211-06818}.)
% }

% \twrchanged{
    The grouping at level $k$ is the \emph{head} of the \protoWCFLOBDD.
    For a given A-connection edge or B-connection edge $c$ from grouping $g_i$ to $g_{i-1}$, the \emph{return tuple} $rt_c$ associated with $c$ consists of the sequence of targets of return edges from $g_{i-1}$ to $g_i$ that correspond to $c$.
% }
\end{definition}

\subsubsection{Structural Invariants}
The structural invariants mainly deal with (i) the organization of return tuples, and (ii) weights in level-0 groupings.
The following invariants deal with constraints on return tuples (and are similar to those for unweighted CFLOBDDs \cite[\S4.1]{DBLP:journals/corr/abs-2211-06818}).
Let $c$ be an A-Connection or B-Connection edge with return tuple $rt_c$ from $g_{i-1}$ to $g_{i}$.
\begin{enumerate}
  \item
    \label{Inv:1}
% If $c$ is an $A$-connection edge, then $rt_c$ must map the exit vertices of $g_{i-1}$ one-to-one, and in order, onto the middle vertices of $g_i$.
     If $c$ is an $A$-connection edge, then $rt_c$ must map $g_{i-1}$'s exit vertices 1-to-1, in order, onto $g_i$'s middle vertices.
  \item
    If $c$ is the $B$-connection edge whose source is middle vertex $j+1$ of $g_i$ and whose target is $g_{i-1}$, then $rt_c$ must meet two conditions:
        \begin{enumerate}
          \item
            \label{Inv:2a}
            It must map $g_{i-1}$'s exit vertices 1-to-1 (but not necessarily onto) $g_i$'s exit vertices.
          \item
            \label{Inv:2b}
% It must ``compactly extend'' the set of exit vertices in $g_i$ defined by the return tuples of the previous $j$ $B$-connections (see \cite[Defn.\ 4.1(2)(b)]{DBLP:journals/corr/abs-2211-06818}).
            Return edges not mapped to exit vertices of $g_i$ that are targets of return tuples of $B$-connections $[1..j]$ must ``compactly extend'' $g_i$'s exit vertices (similar to condition \ref{Inv:1} on A-connections).
            See \cite[Defn.\ 4.1(2)(b)]{DBLP:journals/corr/abs-2211-06818}.
        \end{enumerate}
  \item
    A \protoWCFLOBDD can be used (pointed to by other higher-level groupings) multiple times, but a \protoWCFLOBDD never contains two separate instances of equal {\protoWCFLOBDD}s.
      (Equality is defined inductively on the hierarchical structure of groupings.)
    
  \item
    For every pair of $B$-connections $c$ and $c'$ of grouping $g_i$, with associated return tuples $rt_c$ and $rt_{c'}$, if $c$ and $c'$ lead to two level $i-1$ \protoWCFLOBDD, say $p_{i-1}$ and $p'_{i-1}$, such that $p_{i-1} = p'_{i-1}$, then the associated return tuples must be different (i.e., $rt_c \neq rt_{c'}$).
    \mas{
    The condition means that two $B$-connections $c$ and $c'$ can ``call'' the same \protoWCFLOBDD, but the two sets of return edges $rt_c$ and $rt_{c'}$ have to be different.
    }
\end{enumerate}

The following constraints pertain to the weights associated with edges in level-0 groupings:
\begin{enumerate}
  \item
    The left-edge and right-edge weights $(lw, rw)$ must obey:
    \begin{equation*}
        (lw, rw) = \begin{cases}
        (\bar{1}, rw) & \text{when $lw \neq \bar{0}$}\\
        (\bar{0}, \bar{1}) &\text{ otherwise }
        \end{cases}
    \end{equation*}
  \item
    If a middle vertex $m$ of $g_i$ has a path with aggregated weight $\bar{0}$ from the entry vertex of $g_i$ to $m$, then there must exist an exit-vertex $e$ such that every level-0 grouping edge on every path from $m$ to $e$ has a weight $\bar{0}$.
  \item
    If $e$ is an exit vertex of the topmost-level grouping such that all paths of weight $\bar{0}$ lead to $e$, then $e$ must map to terminal value $\bar{0}$.
    \item If all paths of the WCFLOBDD lead to value $\bar{0}$, then the factor-edge must also have a weight of $\bar{0}$.
\end{enumerate}

% \twrchanged{
In a level-$k$ \emph{WCFLOBDD} $\langle f, G, V \rangle$,
\begin{enumerate}
  \item
    Grouping $G$ heads a level-$k$ \protoWCFLOBDD.
  \item
    Value-tuple $V$ is one of $\{ [\bar{0}], [\bar{1}], [\bar{0}, \bar{1}], [\bar{1}, \bar{0}] \}$, and thus maps each exit vertex of $G$ to a distinct terminal value.
    If there exists an exit vertex $e$ of $G$ such that all paths leading to $e$ have weight $\bar{0}$, then $e$ is mapped to $\bar{0}$.
\end{enumerate}
% }

\subsubsection{Canonicity Theorem}
% Each function from $2^k$ Boolean arguments to a semi-field (equivalently, each decision tree with $2^{2^k}$ leaves and height $2^k$) has a canonical representation as a level-$k$ WCFLOBDD, up to isomorphism.

\begin{theorem}
If $C_1$ and $C_2$ are two level-$k$ WCFLOBDDs for the same Boolean function, and $C_1$ and $C_2$ use the same variable ordering, then $C_1$ and $C_2$ are isomorphic.
\end{theorem}
\begin{ProofSketch}
    We prove the theorem by establishing three properties:
\begin{enumerate}
    \item Every level-$k$ WCFLOBDD represents a decision tree with $2^{2^k}$ leaves.
    \item Every decision tree with $2^{2^k}$ leaves is represented by some level-$k$ WCFLOBDD.
    \item No decision tree with $2^{2^k}$ leaves is represented by more than one level-$k$ WCFLOBDD (up to isomorphism).
\end{enumerate}

\emph{Obligation 1.} We can prove this obligation by induction. Let $P(l)$ represent the number of leaves of a decision tree, 
for the function represented by a level-$l$
% \twrchanged{
\protoWCFLOBDD.
% }
\mas{
We want to prove that $P(l) = 2^{2^l}$.
}
\begin{itemize}
    \item Base Case: $l = 0$, number of variables = 1, number of paths = number of leaves in a decision tree = 2.
    \item Induction Step: Let $P(m) = 2^{2^m}$.
    We wish to prove that $P(m+1) = 2^{2^{m+1}}$.
    Given a level-$l$ \protoWCFLOBDD with head $g_l$, the number of variables of $g_l$ is equally divided between the A-Connection and B-Connections of $g_l$, \mas{by construction}. 
    Hence, for a level-$m{+}1$ \protoWCFLOBDD, we have
    $
      P(m+1) = \sum_{j}A_j(m) \cdot P(m) = (\sum_j A_j(m)) \cdot P(m) =  P(m) \cdot P(m) = 2^{2^m} \cdot 2^{2^m}  = 2^{2^{m+1}}
    $,
    \mas{
    where $A_j(m)$ is the number of matched paths through the level-$m$ A-Connection \protoWCFLOBDD to its $j^{th}$ exit vertex. However, we are just summing over all A-Connection exit vertices, so $\sum_j A_j(m) = P(m)$.
    }
\end{itemize}

\emph{Obligation 2.}
% \twrchanged{
This property is established by giving a (deterministic) procedure to convert a decision tree with $2^{2^k}$ leaves into a level-$k$ WCFLOBDD (satisfying all structural invariants). The construction is given in Appendix~\sectref{canonicalness}.
(The construction is a recursive procedure that works greedily over the decision tree, from left to right.)
% }

\emph{Obligation 3.}
% \twrchanged{
This property is established by unfolding a WCFLOBDD $C$ into a decision tree, folding the decision tree back to a WCFLOBDD $C'$, and showing that $C'$ is isomorphic to $C$.
(The folding-back step uses the same deterministic construction from Obligation 2.)
% }
% algorithm (Appendix~\sectref{canonicalness}) which makes the new WCFLOBDD $C'$ isomorphic to $C$. This proves that there exists only one unique, canonical level-$k$ WCFLOBDD representation of a decision tree with $2^{2^k}$ leaves.
% 
% \emph{Discussion of Construction Algorithm.} The detailed algorithm for constructing a WCFLOBDD from a Decision Tree representation of a function $f$ is given in Appendix~\sectref{canonicalness}. Briefly describing the algorithm, the decision tree $T$ is first converted to a canonical weighted decision tree $T'$ and then WCFLOBDD is constructed from $T'$ by folding $T'$ recursively into a WCFLOBDD \emph{greedily, from left to right}.
\end{ProofSketch}
